Cooperative Perception for Safe Control of Autonomous Vehicles under LiDAR Spoofing Attacks

Autonomous vehicles rely on LiDAR sensors to detect obstacles such as pedestrians, other vehicles, and fixed infrastructures. LiDAR spoofing attacks have been demonstrated that either create erroneous obstacles or prevent detection of real obstacles, resulting in unsafe driving behaviors. In this paper, we propose an approach to detect and mitigate LiDAR spoofing attacks by leveraging LiDAR scan data from other neighboring vehicles. This approach exploits the fact that spoofing attacks can typically only be mounted on one vehicle at a time, and introduce additional points into the victim's scan that can be readily detected by comparison from other, non-modified scans. We develop a Fault Detection, Identification, and Isolation procedure that identifies non-existing obstacle, physical removal, and adversarial object attacks, while also estimating the actual locations of obstacles. We propose a control algorithm that guarantees that these estimated object locations are avoided. We validate our framework using a CARLA simulation study, in which we verify that our FDII algorithm correctly detects each attack pattern.

==> sections/FTAugPer_v1.tex <==
\section{Fault Tolerant Augmented Perception}
data pruning
\subsection{Occupied Area Identification}
observed point projection
occupied 2d convex hull
Def Unsafe region = Convex hull + noise and resolution bounds 
ToDo item: B1 prove the convex hull contains objects
B1: true obstacle's 2D-projection $\subseteq$ unsafe region 

\subsection{Augmented Perception}
algorithm
\subsection{Fault Detection, Identification and Isolation}
decision tree
None-T: no attack, existence of obstacle = T
None-F: no attack, existence of obstacle = F

| Attack  | detect i | Ui non-empty | scan match |% detect j |
| None-T  |   T      |      T       |     T      |%    T     |
| None-F  |   F      |      F       |     -      |%    F     |
|  a      |   T      |      T       |     F      |%    F     |
|  b1,2   |   F      |      T       |     F      |%    T     |
|  b3     |   F      |      T       |     T      |%    T     |
|  c      |   F      |      T       |     T      |%    F     |

Step 1: detect i XOR Ui non-empty (TTTFFF)
        output: T -> No hidden obstacle (all obstacles can be detected even it is a fake obstacle)
                F -> Exist hidden obstacle
Step 2: Scan match
    Branch 1 (None/a): 
        None-F is excluded since it does not have occupied area
        Scan match to distinguish a vs None-T
            ToDo item: A1 proof of correctness
                       A1: Scan match = T -> No relay attack
                           Scan match = F -> Exist relay attack
            
    Branch 2 (b/c):
        Scan match to distinguish b vs c
            ToDo item: A1 proof of correctness
            Output: T -> b3/c  No/cannot observe relay attack area
                    F -> b1/b2 Exist relay attack
                    
        % (Remove) sub-branch (b3/c):
        %     use detect j to distinguish b3/c
        %     detect j T -> b3
        %     detect j F -> c

ToDo item: A2 proof decision tree correctness 
A2: Decision tree can detect fault and identify fault into correct subsets. (Contradiction)

Def Unsafe region = $U_i \cap U_j$ 
ToDo item: B2 prove the overlapping occupied area contains objects
B2: true obstacle's 2D-projection $\subseteq$ unsafe region 

NDT scan match FDII (A1)
Proof of correctness (A2)
Unsafe region (B2)

Process: Pruned data (remove default map info), keep ground info, keep obstacle info
Scan match:
    region: the union of occupied area of agent A and B ($U_A \cup U_B$)
    left: Augmented perception of agent A: observation in $U_A$ $\cup$ processed data from B
    right: Augmented perception of agent B: observation in $U_B$ $\cup$ processed data from A

% A1 tips: 
% squared exponential of L(r) -> convexity
% \theta = min_e' -L(r) 
% Noise bound -> \theta

Observation of A overlap with observation of B ($O_A=\{p_i \mid p_i = obs_i + \mathcal{N}\}$, $O_B$). O.W, none overlapping. 
Agent A is under attack $O_A = e^{\prime}$
Case 1. Exist obstacle (None-T/b3,c), None overlapping $Aug_A = Aug_B$: 
    $Aug_A \ominus Aug_B = ((Ground_A\cap U_B) \cup e^{\prime} \cup (O_B\cup Ground_B\cap U_A))\\ \ominus ((Ground_B\cap U_A)\cup O_B\cup (e^{\prime}\cup Ground_A\cap U_B))$
    We can find the left-hand side of scan match is identical to the right-hand side. Thus, we have NDT result as: $r=0,L(r)=n_s$. 
    
Case 2. Exist obstacle (None-T/c), overlapping:
    In this case we treat the non-overlapping area as Case 1. 
    We take the overlapping area out to analyze. 
    $Aug_A \ominus Aug_B = \\
    O_A \cup O_B \cup (Ground_B \cap U_A) \cup (Ground_A \cap U_B) \ominus O_B \cup (Ground_A \cap U_B) \cup (Ground_B \cap U_A)
    $ 

Case 3. Exist relay attack (a,b1,b2): 
We first consider attack (a), in whose settings, $U_A \neq \emptyset$ and $U_B = \emptyset$
    $Aug_A \ominus Aug_B = \\
    e^{\prime} \cup (Ground_B \cap U_A) \ominus (Ground_B \cap U_A)$
    We next consider b1 and b2. Intuitively, when b1 and b2 happens it means Case1 and Case3(a) happens at the same time. Hence, on both side of the scan match, we have difference caused by $e^{\prime}$ only. 

Case 1/2 LHS=RHS -> no fake obstacle/ cannot observe fake obstacle
Case 3 $e^{\prime} \cup (Ground_B \cap U_A) \ominus (Ground_B \cap U_A)$ causing mis-match

% use intersection instead of union of the occupied areas in scan match
Case 1. Exist obstacle (None-T/b3,c), None overlapping $Aug_A = Aug_B$:
    $Aug_A \ominus Aug_B = \\
    e^{\prime} \cup O_B \ominus e^{\prime} \cup O_B
    $
    LHS = RHS. Thus, we have NDT result as: $r=0,L(r)=n_s$. 

Case 2. Exist obstacle (None-T/c), overlapping:
    In this case we treat the non-overlapping area as Case 1. 
    We take the overlapping area out to analyze. 
    $Aug_A \ominus Aug_B = \\
    e^{\prime} \cup O_B \ominus O_B \cup e^{\prime}
    $
    LHS = RHS. Thus, we have NDT result as: $r=0,L(r)=n_s$.

Case 3. Exist relay attack (a,b1,b2): 
We first consider attack (a), in whose settings, $U_A \neq \emptyset$ and $U_B = \emptyset$
    $Aug_A \ominus Aug_B = \\
    \emptyset \ominus \emptyset
    $
    Cannot do scan match.
    We next consider b1 and b2. Intuitively, when b1 and b2 happens it means Case1 and Case3(a) happens at the same time. The result consists of intersection part and Agent A only part (intersection is empty set). The formal has identical LHS and RHS. The latter cannot do scan match.


==> sections/FTFDII_v1.tex <==
\section{Fault Tolerant FDII}
data pruning

\subsection{Occupied Area Identification}
observed point projection
occupied 2d convex hull
Def Unsafe region = Convex hull + noise and resolution bounds 
ToDo item: B1 prove the convex hull contains objects
B1: true obstacle's 2D-projection $\subseteq$ unsafe region 

\subsection{Augmented Perception}
algorithm

\subsection{Fault Detection, Identification and Isolation}
decision tree
None-T: no attack, existence of obstacle = T
None-F: no attack, existence of obstacle = F

| Attack  | detect i | Ui non-empty | scan match |% detect j |
| None-T  |   T      |      T       |     T      |%    T     |
| None-F  |   F      |      F       |     -      |%    F     |
|  a      |   T      |      T       |     F      |%    F     |
|  b1,2   |   F      |      T       |     F      |%    T     |
|  b3     |   F      |      T       |     T      |%    T     |
|  c      |   F      |      T       |     T      |%    F     |

Step 1: detect i XOR Ui non-empty (TTTFFF)
        output: T -> No hidden obstacle (all obstacles can be detected even it is a fake obstacle)
                F -> Exist hidden obstacle
Step 2: Scan match
    Branch 1 (None/a): 
        None-F is excluded since it does not have occupied area
        Scan match to distinguish a vs None-T
            ToDo item: A1 proof of correctness
                       A1: Scan match = T -> No relay attack
                           Scan match = F -> Exist relay attack
            
    Branch 2 (b/c):
        Scan match to distinguish b vs c
            ToDo item: A1 proof of correctness
            Output: T -> b3/c  No/cannot observe relay attack area
                    F -> b1/b2 Exist relay attack
                    
        % (Remove) sub-branch (b3/c):
        %     use detect j to distinguish b3/c
        %     detect j T -> b3
        %     detect j F -> c

ToDo item: A2 proof decision tree correctness 
A2: Decision tree can detect fault and identify fault into correct subsets. (Contradiction)

Def Unsafe region = $U_i \cap U_j$ 
ToDo item: B2 prove the overlapping occupied area contains objects
B2: true obstacle's 2D-projection $\subseteq$ unsafe region 

NDT scan match FDII (A1)
Proof of correctness (A2)
Unsafe region (B2)

Next step:
Ground data/ Pruned data/ original data ?
Scan match data (?)vs(?) -> T/F

% A1 tips: 
% squared exponential of L(r) -> convexity
% \theta = min_e' -L(r) 
% Noise bound -> \theta

Lemma 1: prove that the occupied area covers the projections of the obstacle.
\begin{enumerate}
    \item Input: observation of the obstacle $\mathcal{O}_b(x,S)$, set of the oblique projections $\mathcal{O}^p(x, S),$ set of points in the obstacle $P_{ob}.$

    \item Output: occupied area $\mathcal{U}$ as the convex hull of $\mathcal{P}(\mathcal{O}_b(x, S)) \cup \mathcal{O}^p(x, S)$
\end{enumerate}

\begin{lemma}
    Given the observation of an obstacle $\mathcal{O}_b(x,S)$, the set of the oblique projections $\mathcal{O}^p(x, S),$ and the set of points in the obstacle $P_{ob}.$ If occupied area $\mathcal{U}$ is computed as the convex hull of the union of $\mathcal{P}(\mathcal{O}_b(x, S))$ and $\mathcal{O}^p(x, S)$, then $\mathcal{P}(P_{ob}) \subseteq \mathcal{U}.$ %the vertical projections of the points of the obstacle are in $\mathcal{U}$.
\end{lemma}


Lemma 2: prove that Attack a, b1, and b2 could be distinguished from the true obstacle, Attack b3, and c.
\begin{enumerate}
    \item Input: attack categories 

    \item Output: whether $(\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \setminus \mathcal{U}_B)$ is empty (based on Lemma 1)
\end{enumerate}

\begin{lemma}
    Suppose Agent A may be under attack and Agent B is safe. If Attack a, b1, or b2 occurs, then $(\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \setminus \mathcal{U}_B) \neq \emptyset.$ If there is a true obstacle or Attack b3 or c occurs, then $(\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \setminus \mathcal{U}_B) = \emptyset.$
\end{lemma}


Theorem 1: prove that the decision tree can classify different attacks
\begin{enumerate}
    \item Input: the observation of obstacle of Agent A $\mathcal{O}_b(x_A, S_A)$, the occupied area of Agent B $\mathcal{U}_B$, the bounding box and classification results of the object detection algorithm of Agent A

    \item Output: the classification of the attack (based on Lemma 2)
\end{enumerate}

\begin{lemma}
    Given the observation of obstacle of Agent A $\mathcal{O}_b(x_A, S_A)$, the occupied area of Agent B $\mathcal{U}_B$, and the bounding box and classification results of the object detection algorithm of Agent A, if the decision tree is executed, then the attack on the observation could be detected and classified once the attack occurs.
\end{lemma}


Theorem 2: prove that the intersection of the occupied areas contains the true unsafe region
\begin{enumerate}
    \item Input: the occupied area of Agent A $\mathcal{U}_A$ and Agent B $\mathcal{B}$

    \item Output: the updated unsafe region (based on Lemma 1)
\end{enumerate}

\begin{lemma}
    If the occupied area of Agent A $\mathcal{U}_A$ and Agent B $\mathcal{B}$ are given, then the updated unsafe region $\mathcal{U}_A \cap \mathcal{B}$ contains the true unsafe region $\mathcal{P}(P_{ob})$.
\end{lemma}

==> sections/FTSafeControl_v1.tex <==
\section{Hybrid System Safe Control}
Hybrid model
safety proof

==> sections/Formulation.tex <==
\section{Formulation}
\subsection{System Model}
Consider a discrete-time control-affine system given as:
\begin{equation}
    \label{eq:dynamic}
    x[k+1] = f(x[k]) + g(x[k]) u[k]
    % x[k+1] = f(x[k]) + g(x[k]) u[k] + w[k]
\end{equation}
where $w[k]$ is a Gaussian process with mean  zero and autocorrelation function $R_{w}(k,k^{\prime}) = Q_{k}\delta(k-k^{\prime})$ with $\delta$ denoting the discrete-time delta function and $Q_{k}$ is a positive definite matrix.  

\iffalse
Bicycle dynamics \cite{kong2015kinematic}
\begin{equation}
\begin{aligned}
\ddot{x} & =\dot{\psi} \dot{y}+a_x \\
\ddot{y} & =-\dot{\psi} \dot{x}+\frac{2}{m}\left(F_{c, f} \cos \delta_f+F_{c, r}\right) \\
\ddot{\psi} & =\frac{2}{I_z}\left(l_f F_{c, f}-l_r F_{c, r}\right) \\
\dot{X} & =\dot{x} \cos \psi-\dot{y} \sin \psi \\
\dot{Y} & =\dot{x} \sin \psi+\dot{y} \cos \psi
\end{aligned}
\end{equation}
\fi

We let $x[k]\in \mathcal{X} \subseteq \mathbb{R}^n$ denote the system state and $u[k] \in \mathbb{R}^m$ denote a control signal at time $k$. Functions $f:\mathbb{R}^n\rightarrow\mathbb{R}^n$ and $g:\mathbb{R}^{n}\rightarrow\mathbb{R}^{n\times m}$ are assumed to be Lipschitz continuous.

% System \eqref{eq:dynamic} uses a set of sensors $I_p:=\{1,\ldots,n_{p}\}$ to measure its states with observation $y[k] \in \mathbb{R}^{z}$ following the dynamics described as:

\begin{equation}
    \label{eq:observation}
    y[k] = o(x[k]) + v[k],
\end{equation}
where $o:\mathbb{R}^n\rightarrow\mathbb{R}^z$ is the observation function, $v[k]$ is an independent Gaussian process with mean identically zero and autocorrelation function $R_{v}[k,k^{\prime}] = R_{k}\delta(k-k^{\prime})$ and $R_{k}$ is a positive definite matrix. 

A LiDAR sensor fires and collects $n_s$ laser beams and calculate the ranges and angles to objects. Specifically, we let $p_i := (s^r_i, s^a_i)$ for 2-D LiDAR and $p_i := (s^r_i, s^a_i, s^{\phi}_i)$ for 3-D LiDAR, where $s_i^r$ denotes the range, $s_i^a$ denotes the horizontal angle and $s^{\phi}_i$ denotes vertical angle of the $i$-th scan. It observes the environment by constructing a scan, i.e. $S:=\{p_i,\ 0\leq i\leq n_s\}$. We let $\mathcal{P}_i$ to denote the corresponding area covered by point $p_i \in S$. We denote the Cartesian translated LiDAR scan $S$ measured at pose $x$ as $\mathcal{O}(x,S)$. Let the scan covered area of the observation denoted as $\mathcal{I}$. We let $\mathcal{U}$ to denote the occupied area within LiDAR measurement range. 

\subsection{Threat Model}
\label{subsec:threat-model}
In this paper, we consider attacks with different purposes, namely falsifying obstacles and hiding obstacles. To falsify obstacles, the adversary conduct relay perturbations by firing laser beams to inject several artificial points $e^{\prime}$ into a LiDAR scan. We denote the compromised LiDAR scan as $S \oplus e^{\prime}$, where $\oplus$ is a merge function introduced by \cite{cao2019adversarialsen}. To hide obstacles, the attacker can either synthesize adversarial obstacles~\cite{cao2019adversarialobj} as hidden obstacles or conduct physical removal attacks~\cite{cao2022you} by injecting false data to overwrite arbitrary object. However, due to the physical limitation of spoofer hardware, the injected point can only be within a very narrow spoofing angle, i.e. less than $10^{\circ}$ horizontal angle. Hence, in this paper, we assume that one attacker can only spoof one LiDAR sensor. 

We denote the area affected by spoofer as $\varepsilon$. We assume the affected area $\varepsilon$ of attack $e^{\prime}$ on victim agent $i$ is overlapped by other agents' observation area. Specifically, there exists a non-empty set $L$ such that 
\begin{equation}
    \label{eq:jointpercept}
    \varepsilon \subset \mathcal{I}_{i} \cap \bigcup_{j\neq i, j\in L \subseteq \{1,\ldots,n_A\}} \mathcal{I}_j
\end{equation}
% We assume there exist $n_A > 1$ agents whose measurements overlap the spoofed data
% Specifically, there exist some $i,j$ such that
% \begin{equation}
%     \label{eq:jointpercept}
%     \varepsilon \subset \bigcap_{i,j}\mathcal{O}(x_i,S_i), 
% \end{equation}
% where $i \neq j$ and $i,j\in\{1,\ldots,n_A\}$. 

\subsection{Safety and Problem Fomrulation}
We define the safety set $\mathcal{C}$ as  
\begin{equation*}
    \mathcal{C}= \{x\in\mathcal{X}:h(x)\geq0\},
\end{equation*}
where $h:\mathcal{X}\mapsto\mathbb{R}$. We say system \eqref{eq:dynamic} is safe with respect to $\mathcal{C}$ if $x[k]\in\mathcal{C}$ for all time $k= 0,1,\ldots$. Note that, we do not assume knowing the accurate map or exact safety region. The safety set is synthesized from LiDAR observation. We denote the synthesized safety set as $\mathcal{D}$. However, due to the existence of malicious attacker, synthesized safety set may not be correct, i.e. $\mathcal{D}\subseteq \mathcal{C}$. 

\begin{problem}
\label{prob:main}
We consider $n_A$ nonlinear LiDAR-based systems with dynamics \eqref{eq:dynamic} such that \eqref{eq:jointpercept} holds. The problem studied is to find a scheme to estimate safety region and ensure system safety with desired probability $(1-\delta)$, where $\delta\in(0,1)$, when an adversary is present. 
\end{problem} 

\subsection{Preliminaries}
In what follows, we give background on discrete-time Extended Kalman Filter (EKF) and estimating pose from LiDAR scans

\subsubsection{DT-EKF}
For the system with dynamics \eqref{eq:dynamic} and observation \eqref{eq:observation}, the state estimate $\hat{x}$ is computed via EKF as:
\begin{equation}
\label{eq:dt-ekf}
    \hat{x}[k+1] = F(\hat{x}[k], u[k]) + K_k(y[k] - o(\hat{x}[k])),
\end{equation}
where $F(x[k],u[k])= f(x[k]) + g(x[k]) u[k]$.
The Kalman filter gain is 
\begin{equation}
\label{eq:ekfgain}
    K_k = A_{k} P_{k} C_{k}^{T}(C_{k} P_{k} C_{k}^{T}+R_{k})^{-1},
\end{equation}
where $A_{k} =\frac{\partial F}{\partial x}(\hat{x}[k], u[k]) $,   $C_{k} =\frac{\partial o}{\partial x}(\hat{x}[k])$, and $P_k$ is defined by the Riccati difference equation:
\begin{equation*}
    P_{k+1}=A_{k} P_{k} A_{k}^{T}+Q_{k}-K_{k}(C_{k} P_{k} C_{k}^{T}+R_{k}) K_{k}^{T}. 
\end{equation*}

The error bound of discrete-time EKF can be derived by Theorem 3.2 in \cite{reif1999stochastic} if Assumption \ref{assump:dtekf} holds.

\begin{assumption}
\label{assump:dtekf}
The system described by \eqref{eq:dynamic} and \eqref{eq:observation} satisfies the conditions: 
\begin{itemize}
    \item $A_{k}$ is nonsingular for every $k \geq 0$.
    \item There are positive real numbers $\bar{a}, \bar{c}, \underline{p}, \bar{p}>0$ such that the following bounds on various matrices are fulfilled for every $k \geq 0$ :
    \begin{equation*}
        \begin{aligned}
        &\left\|A_{k}\right\| \leq \bar{a}; \
        \left\|C_{k}\right\| \leq \bar{c}; \
        \underline{p} I \leq P_{k} \leq \bar{p} I; \\
        &\underline{q} I \leq Q_{k}; \ 
        \underline{r} I \leq R_{k} .
        \end{aligned}
    \end{equation*}
    \item Let $\phi$ and $\chi$ be defined as
    \begin{align*}
        &F(x[k],u[k]) - F(\hat{x}[k],u[k]) = A_k (x[k]-\hat{x}[k]) \\
        &\quad\quad\quad\quad\quad\quad\quad\quad+ \varphi(x[k], \hat{x}[k], u[k]) \\
        &o(x[k])-o(\hat{x}[k]) =C_{k}(x[k]-\hat{x}[k])+\chi(x[k], \hat{x}[k])
    \end{align*}
    Then there are positive real numbers $\epsilon_{\varphi}, \epsilon_{\chi}, \kappa_{\varphi}, \kappa_{\chi}>0$ such that the nonlinear functions $\varphi, \chi$ are bounded via
    % $$
    % \begin{aligned}
    % \|\varphi(x, \hat{x}, u)\| & \leq \kappa_{\varphi}\|x-\hat{x}\|^{2} \\
    % \|\chi(x, \hat{x})\| & \leq \kappa_{\chi}\|x-\hat{x}\|^{2}
    % \end{aligned}
    % $$
    \begin{equation*}
        \|\varphi(x, \hat{x}, u)\|  \leq \kappa_{\varphi}\|x-\hat{x}\|^{2},\quad
    \|\chi(x, \hat{x})\|  \leq \kappa_{\chi}\|x-\hat{x}\|^{2}
    \end{equation*}
    for $x, \hat{x} \in R^{n}$ with $\|x-\hat{x}\| \leq \epsilon_{\varphi}$ and $\|x-\hat{x}\| \leq \epsilon_{\chi}$, respectively.
\end{itemize}

\end{assumption}

If the conditions of Assumption 1 hold, the estimation error $\zeta_{k}=x[k]-\hat{x}[k]$ is exponentially bounded in mean square and bounded with probability one, provided that the initial estimation error satisfies $\left\|\zeta_{0}\right\| \leq \Bar{\zeta}$ \cite{reif1999stochastic}. 

\subsubsection{Comparing Scans}
Pose refers to the position of the system in a Cartesian coordinate frame. Pose estimations with LiDAR scans have been extensively studied. NDT~\cite{biber2003normal}, as one of the widely-used approaches, models the distribution of all reconstructed 2D-Points of one laser scan by a collection of local normal distributions. 

Consider two states $x_1,x_2\in\mathcal{X}$ and the LiDAR scans $\mathcal{O}(x_1,S_1)$ and $\mathcal{O}(x_2,S_2)$ collected at $x_1$ and $x_2$, respectively. The NDT method estimates the relative pose change as $r=\mathcal{O}(x_1,S_1) \ominus \mathcal{O}(x_2,S_2)$, where $\ominus$ is a scan match operation.
% Define $r:=x_2-x_1$ as relative pose change of two LiDAR observations $\mathcal{O}(x_1,S_1)$ and $\mathcal{O}(x_2,S_2)$. 
% We further define the NDT method to estimate relative pose as an scan match operation denoted as $\ominus$ and formulated as
% \begin{equation}
% \label{eq:ndt_opt}
%     r = \mathcal{O}(x_1,S_1) \ominus \mathcal{O}(x_2,S_2).
% \end{equation}
The scan match operation is implemented as follows. The NDT method first subdivides the surrounding space uniformly into cells with constant size. For each cell in $\mathcal{O}(x_1,S_1)$, the mean $q$ and the covariance matrix $\Sigma$ are computed to model the points contained in the cell as the normal distribution $N(q, \Sigma)$. 
Denote the points in $\mathcal{O}(x_2,S_2)$ as $p_i,\ i\in n_s$, where $p_i$ is a position vector and $n_s$ is the number of valid points.
% A frame of a LiDAR scan denoted as $S$ is a set of $n_p$ points $\{p_{i=1 . . n_p}\}$ of obstacle position collected by one laser scan. 
% Define $r:=x2-x1$ as relative pose change of two LiDAR observations $\mathcal{O}(x_1,S_1)$ and $\mathcal{O}(x_2,S_2)$. 
Define loss function $\mathcal{L}_s(r^{\prime})$ as
\begin{equation}
    \label{eq:score}
    \mathcal{L}_s(r^{\prime}) = \sum_{i} \exp \left(\frac{-((p_i-r^{\prime})-{q}_{i})^{T} {\Sigma}_{i}^{-{1}}((p_i-r^{\prime})-{q}_{i})}{2}\right)
\end{equation}
The relative pose change $r^{\prime}$ is estimated by solving the minimization problem
% Estimating $r^{\prime}$ is to solve the minimization problem: 
\begin{equation}
\label{eq:ndt_obj}
    \min_{r^{\prime}}{-\mathcal{L}_s(r^{\prime})}
\end{equation}
with Newton's algorithm. We use $r$ to denote the solution to \eqref{eq:ndt_obj} for the rest of the paper. The corresponding loss $\mathcal{L}_s(r)$ can be computed with the output of scan match $r$ by \eqref{eq:score}. 

==> sections/ProposedMethod.tex <==
\section{Proposed Method}
In this section we propose a fault tolerant augmented perception to obtain an accurate environmental estimation. The proposed approach is illustrated as Fig.~\ref{fig:illustration}.

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figs/illustration.png}
    \caption{Schematic illustration of the proposed approach.}
    \label{fig:illustration}
\end{figure}

\subsection{Occupied Area Identification}
In this subsection, we present the method to identify and extract the occupied area $\mathcal{U}$, and transmit it to the augment perception and FDII components.

We prune the raw data $\mathcal{O}(x, S)$ by removing the points corresponding to the infrastructure (eg. wall) on a default map. For the rest of the paper, we use $\mathcal{O}(x, S)$ to denote the pruned raw data without infrastructure. %The remaining points 

We define the vertical projection operation $\mathcal{P}(\mathcal{O})\longrightarrow \mathcal{Y},$ which takes an observation $\mathcal{O}$ as input and outputs the set $\mathcal{Y}$ of the projections of the points in $\mathcal{O}$. %Denote the set of points corresponding to the obstacles as $\mathcal{O}_\mathcal{O}(x,S) := \{p=(o^x, o^y, o^z), o^z > \zeta^z\}$.
We let $\mathcal{U}$ to denote the occupied area within LiDAR measurement range. 

We utilize the altitude coordinates of the points to distinguish the ground and the obstacle. For point $o_i = (o^x_i, o^y_i, o^z_i)$ in $\mathcal{O}(x, S),$ $\forall i \in n_s,$ if $o^z_i \leq \zeta^z,$ then the corresponding area $\mathcal{A}_i$ is contained by the ground. If $o^z_i > \zeta^z,$ then $\mathcal{A}_i$ is contained by the obstacle, where $\zeta^z$ is the estimation error of the altitude coordinates. There exist ground removal approaches that use this scheme to remove ground from 3D scan~\cite{qian2014ncc}\cite{bogoslavskyi2017efficient}.

After ground removal, we get the observation of points corresponding to the obstacle $\mathcal{O}_\mathcal{O}(x,S) := \{p=(o^x, o^y, o^z), o^z > \zeta^z\}$. %Denote the average of the points in $\mathcal{O}^o(x, S)$ as $\Bar{o}$, and the maximum distance between the points in $\mathcal{O}^o(x, S)$ and $\Bar{o}$ as $d = \max \|\|$
We further calculate the oblique projections of the points in $\mathcal{O}_\mathcal{O}(x, S)$ from LiDAR to the ground and denote the set of the oblique projections as $\mathcal{O}^p(x, S).$ These projections are calculated via similar triangles. The occupied area $\mathcal{U}$ is computed as the convex hull of the union of $\mathcal{P}(\mathcal{O}_\mathcal{O}(x, S))$ and $\mathcal{O}^p(x, S)$. The convex hull can be calculated via open-source tools such as Scipy~\cite{virtanen2020scipy}.

\begin{lemma}
    Given the observation of an obstacle $\mathcal{O}_\mathcal{O}(x,S)$ and the the set of the oblique projections $\mathcal{O}^p(x, S).$ If occupied area $\mathcal{U}$ is computed as the convex hull of the union of $\mathcal{P}(\mathcal{O}_\mathcal{O}(x, S))$ and $\mathcal{O}^p(x, S)$, then the vertical projections of the points of the obstacle are in $\mathcal{U}$.
\end{lemma}

\begin{proof}
    Suppose there is a point $p = (s^r, s^a, s^{\phi})$ of the obstacle. Without loss of generality, we set $s^a = a$ and $s^{\phi} = \phi$. We consider two cases, namely (i) there is line-of-sight between the LiDAR and $p$, and (ii) there is no line-of-sight between the LiDAR and $p.$

    \textit{Case (i):} In this case, $p \in \mathcal{O}_\mathcal{O}(x,S).$ The vertical projection $\mathcal{P}(p) \in \mathcal{P}(\mathcal{O}_\mathcal{O}(x, S)),$ and will be included in the convex hull of the union of $\mathcal{P}(\mathcal{O}_\mathcal{O}(x, S))$ and $\mathcal{O}^p(x, S)$. Thus, $\mathcal{P}(p) \in \mathcal{U}.$

    \textit{Case (ii):} In this case, $p \notin \mathcal{O}_\mathcal{O}(x,S).$ There exists at least one point $p^{\prime}$ in $\mathcal{O}_\mathcal{O}(x,S)$ 
\end{proof}

\subsection{Augmented Perception}
The intuition is to utilize redundant information contained in the LiDAR observations of other agents. To do so, we introduce augmented perception. %Given a fixed Cartesian coordinate with origin $O_c$. 
For each agent indexed, we augment its perception by merging LiDAR observations of other agents $j\in L$. Specifically, we have the augmented scan represented as $S_i \oplus\boldsymbol{S}$, where $\boldsymbol{S}:=\{\bigcup_{j\neq i,j\in L}S^i_j\})$ and the augmented observation $\Tilde{\mathcal{O}}_i(x_i, S_i \oplus\boldsymbol{S})$ centered at $x_i$, where $S^i_j$ is the translated scan $S_j$ under Agent $i$'s coordinate. 

We propose Algorithm \ref{alg:AugPerception} to collect the augmented perception. 

\begin{algorithm}[!htbp]
\caption{Augmented Perception}
\begin{algorithmic}[1]
    \State \textbf{Input:} state estimate $\hat{x}_i$ of agent $i$, a set of nearby agent $L$, a set of state estimate $\hat{x}_j$, $\forall j\in L$, a set of LiDAR observation $\mathcal{O}_j(x_j, S_j)$, $\forall j\in L$
    \State \textbf{Output:} A set of augmented LiDAR Observation $\boldsymbol{\Tilde{\mathcal{O}}}:=\{\Tilde{\mathcal{O}},\forall i\in L\}$
    \For{$i \in L$}
        % \State Set relative pose $r^{\prime}\gets O_c-\hat{x}_i$
        % \State $p_i\gets p_i+r^{\prime}$, $\forall p_i \in \Tilde{\mathcal{O}}_i(x_i,S_i)$ denoted as $\Tilde{\mathcal{O}}_i(O_c,S_i) $
        \For{$j\neq i, j\in L$}
            \For{$\mathcal{P}_k\in(\mathcal{I}_j \cap \mathcal{U}_i)$}
            % \State Transfer point $\Tilde{p}_k \gets  p_k + \hat{x}_i-\hat{x}_j$
            \State Transfer point $\Tilde{p}_k \in S^i_j$ from $p_k in S_j$  
            \State $\Tilde{S}_i \gets S_i \cup \Tilde{p}_k$
            \State Augment perception $\Tilde{\mathcal{O}}_i(x_i,\Tilde{S}_i)$
            \EndFor
        \EndFor
    \EndFor
\end{algorithmic}
\label{alg:AugPerception}
\end{algorithm}

\subsection{Fault Detection, Identification and Isolation}
\label{sec:FDII}
The objective of the proposed fault detection, identification, and isolation (FDII) algorithm is to detect the mismatch between the augmented observations of different agents, identify the spoofed agent, isolate the corrupted parts of the raw data, and restore the true unsafe region. The proposed FDII algorithm is illustrated as Fig.~\ref{fig:FDII}.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figs/decision_tree.png}
    \caption{Decision tree of the FDII algorithm.}
    \label{fig:FDII}
\end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{ |c|c|c|c| } 
     \hline
     Type of Attack & detect i & $U_i$ Non-Empty & Scan Match \\ 
     \hline
     None True & T & T & T \\ 
     None False & F & F & - \\ 
     a & T & T & F \\ 
     b1, b2 & F & T & F \\ 
     b3, c & F & T & T \\
     \hline
    \end{tabular}
    \caption{Decision Table}
    \label{tab:my_label}
\end{table}

The intuition is that if the LiDAR observation of an agent is spoofed by the adversary, the measured point $e^{\prime}$ in spoofed area $\varepsilon$ will not match the data collected by other agent $b\neq a$, $b\in L$. We limit the scope of scan match of the observation to the union of the occupied areas $\mathcal{U}_a\cup \mathcal{U}_b$ of two augmented observation $\Tilde{\mathcal{O}}_a^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_b^{\mathcal{I}}$. 
We also limit the scope of scan match of the observation to the horizontal axes of two augmented observation $\Tilde{\mathcal{O}}_a^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_b^{\mathcal{I}}$. 
% If it is a 2-D LiDAR, we use $\Tilde{\mathcal{O}}_i^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_j^{\mathcal{I}}$. If it is a 3-D LiDAR, we use the values of x and y coordinates of $\Tilde{\mathcal{O}}_i^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_j^{\mathcal{I}}$, which means the projection of the scan on the horizontal plane. 

The following lemma guarantees the detection of the mismatch between observations even if the spoofer presents.

\begin{lemma}
Suppose the object detection algorithms of Agent A outputs the bounding boxes $\mathcal{B}_A$ and the obstacle set $\mathcal{O}_\mathcal{O}(x_A, S_A)$ inside $\mathcal{B}_A$. Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied areas $\mathcal{U}_A$ and $\mathcal{U}_B$ of Agent A and Agent B, respectively, and the obstacle set $\mathcal{O}_\mathcal{O}(x_A, S_B)$ which has $\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B)) \subseteq \mathcal{U}_A$. If $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then there exists a true obstacle in $\mathcal{B}_A$. Otherwise, Agent A is under Attack a. 
% Suppose the object detection algorithms of Agent A outputs the bounding boxes $\mathcal{B}_A$. Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied area $\mathcal{U}_A$ and $\mathcal{U}_B,$ the sets of projection of the points inside $\mathcal{B}_A$ on the horizontal plane $O_A,$ and the set of projection of $O_B$, If the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ match, then there exists a true obstacle
% Suppose the object detection algorithms of Agent A and B output the bounding boxes $\mathcal{B}_A$ and $\mathcal{B}_B$ for the same obstacle, respectively. Given the sets of projection of the points inside $\mathcal{B}_A$ and $\mathcal{B}_B$ on the horizontal plane $O_A$ and $O_B$, the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, and the occupied area $\mathcal{U}_A$ and $\mathcal{U}_B.$ If the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ match, then there exists a true obstacle

\end{lemma}

\begin{proof}
We consider two cases, namely (i) there exists a true obstacle in $\mathcal{B}_A$ and (ii) there exists a falsified obstacle.

\textit{Case (i):} In this case, the spoofer does not present. We calculate the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate as follow.
\begin{align*}
    \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \\
    &\cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
    \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B))\\
    &\cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
\end{align*}

Since $\Tilde{\mathcal{O}}(x_A, S_A) = \Tilde{\mathcal{O}}(x_A, S_B),$ we have $r = 0$ and $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s.$

\textit{Case (ii):} In this case, Agent A is under Attack a and we have $\mathcal{U}_A \neq \emptyset$ and $\mathcal{U}_B = \emptyset.$ Since there is only one attack, Agent B is attack-free and $\mathcal{O}_\mathcal{O}(x_A, S_B) = \emptyset.$ The augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
\begin{align*}
    \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \\
    &\cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
    =& \{\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A))\cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
    \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B))\\
    &\cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}\\
    =&\{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}
\end{align*}

Since $\Tilde{\mathcal{O}}(x_A, S_A) \neq \Tilde{\mathcal{O}}(x_A, S_B),$ the extra term $\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A))$ in $\Tilde{\mathcal{O}}(x_A, S_A)$ will introduce difference in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$

% \textit{Case (i):} In this case, the spoofer does not present. We calculate the scan match $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B)$ as follow.
% \begin{align*}
%     &\quad\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \\
%     &= \{((\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_\mathcal{B}(x_A, S_A)) \\
%     &\quad\cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A))\}\\ 
%     &\ominus ((Ground_B\cap U_A)\cup O_B\cup (e^{\prime}\cup Ground_A\cap U_B))
% \end{align*}
\end{proof}


\begin{lemma}
Suppose there exists the obstacle set $\mathcal{O}_\mathcal{O}(x_A, S_A)$ with the occupied area $\mathcal{U}_A$, and the object detection algorithms of Agent A does not detect any obstacle with vertical projection in $\mathcal{U}_A$.
Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied areas $\mathcal{U}_A$ and $\mathcal{U}_B$ of Agent A and Agent B, respectively, and the obstacle set $\mathcal{O}_\mathcal{O}(x_A, S_B)$ which has $\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B)) \subseteq \mathcal{U}_A$. If $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then there exists Attack b3 or Attack c which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$. Otherwise, there exists Attack b1 or Attack b2 which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$. 
\end{lemma}

\begin{proof}
We consider two cases, namely (i) there exists Attack b3 or Attack c which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$, and (ii) there exists Attack b1 or Attack b2 which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$.

\textit{Case (i):} In this case, $\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \subseteq \mathcal{U}_B$ and $\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B)) \subseteq \mathcal{U}_A$. We calculate the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate as follow.
\begin{align*}
    \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \\
    &\cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
    \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B))\\
    &\cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
\end{align*}

Since $\Tilde{\mathcal{O}}(x_A, S_A) = \Tilde{\mathcal{O}}(x_A, S_B),$ we have $r = 0$ and $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s.$

\textit{Case (ii):} In this case, $\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B)) \subseteq \mathcal{U}_A$. However, $\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A))$ is not a subset of $\mathcal{U}_B$, which means that there exist elements in $\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A))$ that is also elements in $\mathcal{I}_B \setminus \mathcal{U}_B$. The augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
\begin{align*}
    \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \\
    &\cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
    \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_B))\\
    &\cup (\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B ) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
\end{align*}

Since there exist elements in $\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A))$ that is not in $\mathcal{U}_B$, we have $(\mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \subseteq \mathcal{P}(\mathcal{O}_\mathcal{O}(x_A, S_A))$ and there are more points in $\Tilde{\mathcal{O}}(x_A, S_A)$ than in $\Tilde{\mathcal{O}}(x_A, S_B)$. This will introduce difference in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$
\end{proof}


We consider three LiDAR attacks presented in Sec.~\ref{subsec:threat-model} as shown in Fig.~\ref{fig:three-LiDAR-attacks}. Without loss of generality, we show the idea by using two agents.

The following lemma shows that the unsafe region can be achieved even if the three LiDAR attacks occur.

\begin{lemma}
    decision tree
\end{lemma}

Based on the results of Lemma ..., we propose the function ... in Algorithm~... to generate unsafe regions that can be used to provide feasible control inputs to guarantee safety requirements.

The rules to update unsafe regions based on multi-agent observations.
\begin{enumerate}
    \item If an occupied area is only observed by one agent, then it covers a falsified non-existing obstacle resulted from a relay attack.

    \item If an occupied area 
\end{enumerate}

Only consider the intersection of occupied area when doing mismatch detection.
\begin{enumerate}
    \item For attack a and b1 (non-existing obstacle), the intersection is empty.

    \item For attack b2 (Agent j could partically observe the area covered by Agent i's occupied area), we could narrow the range of the intersection based on the observation of Agent j.

    \item For attack b3 and c (Agent j cannot observe the area covered by Agent i's occupied area), we append the intersection into the updated unsafe region.
\end{enumerate}

Challenges:
\begin{enumerate}
    \item How to identify the occupied area?

    Divide the overlapping area of the observations $\Tilde{\mathcal{O}}_i(O_c,S_i)$ and $\Tilde{\mathcal{O}}_j(O_c,S_j)$ uniformly into small cells with constant size. If there is no point $p_i$ inside the cell, we consider the empty cell as a part of an occupied area of Agent $i$. The nearby empty cells combine together as an occupied area. The adjacent nonempty cells are considered as the boundary of the occupied area.

    \item How to do augmented perception?

    Do not need augmented perception in this case.

    \item How to do mismatch detection?

    Do not need to do mismatch detection in this case. 
\end{enumerate}

In Fig.~\ref{fig:RelayExp}, the spoofer falsifies a non-existing obstacle in the raw data of the attacked Agent $i$ by firing laser beams to the receiver of the LiDAR. The augment perception $\Tilde{\mathcal{O}}_i(O_c,\Tilde{S}_i)$ of Agent $i$ is obtained by combining points $\Tilde{p}_k$ in the overlapping area of the falsified occupied area $\mathcal{U}_i$ and the scan covered area $\mathcal{I}_j$. This overlapping area is guaranteed to exist and be the same as $\mathcal{U}_i$ by Eq.~\eqref{eq:jointpercept}. The augment perception $\Tilde{\mathcal{O}}_j(O_c,\Tilde{S}_j)$ of Agent $j$ is identical with the observation $\Tilde{\mathcal{O}}_j(O_c,S_j)$ because there is no occupied area in the raw data. Thus, there is mismatch of the observation in the overlapping area $\mathcal{I}_i\cap \mathcal{I}_j$ of two augmented observation $\Tilde{\mathcal{O}}_i^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_j^{\mathcal{I}}$.

In Fig.~\ref{fig:PRAExp}, the spoofer implements PRA by creating a falsified obstacle between Agent $i$ and the true obstacle. Since the position of the falsified obstacle and the position of the true obstacle are different, there exists occupied area that can only be detected by one of the agent, which means $\mathcal{U}_i \neq \mathcal{U}_j$. According to Eq.~\eqref{eq:jointpercept}, $\mathcal{U}_i \subseteq \mathcal{I}_j$ and $\mathcal{U}_j \subseteq \mathcal{I}_i.$ Thus, $(\mathcal{I}_j \cap \mathcal{U}_i) = \mathcal{U}_i \neq \mathcal{U}_j = (\mathcal{I}_i \cap \mathcal{U}_j)$.

In Fig.~\ref{fig:AdvObjExp}, 

We compute relative pose by performing scan match $\Tilde{\mathcal{O}}_i^{\mathcal{I}} \ominus \Tilde{\mathcal{O}}_j^{\mathcal{I}}$. 

\begin{proposition}
    (Working on *proposition)
\end{proposition}
If the relative pose exceed a threshold derived by (*proposition), it means one of the scans is spoofed. We next identify the area affected spoofed data by solving the following optimization problem  
\begin{equation}
    \label{eq:FIdent}
    \min_c (\Tilde{\mathcal{O}}_i^{\mathcal{I}} \backslash c)\ominus (\Tilde{\mathcal{O}}_j^{\mathcal{I}} \backslash c)
\end{equation}
With the mismatched area spotted, we then formulate decision tree to identify the attack type and spoofed agent. 

(working on) train of thought: We summarize the symptom of different attack type and formulate the Decision tree 

\begin{figure}[!htbp]
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width = \textwidth]{figs/FalsifyAttack.jpg}
  \subcaption{Relay attacks falsify non-existing obstacle but leave some trace in the raw data. }
  \label{fig:RelayExp}
\end{subfigure}%
\vfill
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width = \textwidth]{figs/PhysicalRemovalAttack.jpg}
  \subcaption{Physical removal attacks hide object from LiDAR detector but leave some trace in the raw data. }
  \label{fig:PRAExp}
\end{subfigure}%
\vfill
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width = \textwidth]{figs/AdvObjExp.jpg}
  \subcaption{Adversarial objects can hide from LiDAR detector but leave some trace in the raw data. }
  \label{fig:AdvObjExp}
\end{subfigure}%
\caption{Trace in raw data}
\label{fig:three-LiDAR-attacks}
\end{figure}

We finally proposed Alg. \ref{alg:FDII} to summarize the workflow. 
% \begin{algorithm}[!htbp]
% \caption{LiDAR Fault Detection, Identification and Isolation}
% \begin{algorithmic}[1]
%     \State \textbf{Input:} A set of augmented LiDAR Observation $\boldsymbol{\Tilde{\mathcal{O}}}:=\{\Tilde{\mathcal{O}},\forall i\in L\}$
%     \State \textbf{Output:} 
%     \For{$i,j\in L$}
%         \State Compute $r \gets \Tilde{\mathcal{O}}_i^{\mathcal{I}} \ominus \Tilde{\mathcal{O}}_j^{\mathcal{I}}$
%         \If{$r>\theta$}
%             \State Solve \eqref{eq:FIdent}
%             \State (Working on)
%         \EndIf
%     \EndFor
% \end{algorithmic}
% \label{alg:FDII}
% \end{algorithm}


% \subsection{Safety Region Estimation}
\subsection{Safe Control}
% \input{sections/control.tex}
\input{sections/control_v1.tex}
% We next design a safe control methodology to ensure safety of the controlled agent with desired probability. We formulate it as a control of a hybrid system. 

% In section \ref{sec:FDII}, we detect and estimate the obstacle to acquire unsafe region $h_1(x)$. Hence, we have the safe set as $\mathcal{C}_1:=\{x\mid h_1(x)\geq0\}$. 

==> sections/ProposedMethod_v1.tex <==
\newpage
\section{Proposed Method}



In this section we propose a fault tolerant augmented perception to obtain an accurate environmental estimation. The proposed approach is illustrated as Fig.~\ref{fig:illustration}.

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figs/illustration.png}
    \caption{Schematic illustration of the proposed approach.}
    \label{fig:illustration}
\end{figure}

\subsection{Occupied Area Identification}
In this subsection, we present the method to identify and extract the occupied area $\mathcal{U}$, and transmit it to the augment perception and FDII components.

We prune the raw data $\mathcal{O}(x, S)$ by removing the points corresponding to the infrastructure (eg. wall) on a default map. For the rest of the paper, we use $\mathcal{O}(x, S)$ to denote the pruned raw data without infrastructure. %The remaining points 

We define the vertical projection operation $\mathcal{P}(\mathcal{O})\longrightarrow \mathcal{Y},$ which takes an observation $\mathcal{O}$ as input and outputs the set $\mathcal{Y}$ of the projections of the points in $\mathcal{O}$. %Denote the set of points corresponding to the obstacles as $\mathcal{O}_b(x,S) := \{p=(o^x, o^y, o^z), o^z > \zeta^z\}$.
We let $\mathcal{U}$ to denote the occupied area within LiDAR measurement range. 

We utilize the altitude coordinates of the points to distinguish the ground and the obstacle. For point $o_i = (o^x_i, o^y_i, o^z_i)$ in $\mathcal{O}(x, S),$ $\forall i \in n_s,$ if $o^z_i \leq \zeta^z,$ then the corresponding area $\mathcal{A}_i$ is contained by the ground. If $o^z_i > \zeta^z,$ then $\mathcal{A}_i$ is contained by the obstacle, where $\zeta^z$ is the estimation error of the altitude coordinates. There exist ground removal approaches that use this scheme to remove ground from 3D scan~\cite{qian2014ncc}\cite{bogoslavskyi2017efficient}.

After ground removal, we get the observation of points corresponding to the obstacle $\mathcal{O}_b(x,S) := \{p=(o^x, o^y, o^z), o^z > \zeta^z\}$. %Denote the average of the points in $\mathcal{O}^o(x, S)$ as $\Bar{o}$, and the maximum distance between the points in $\mathcal{O}^o(x, S)$ and $\Bar{o}$ as $d = \max \|\|$
We further calculate the oblique projections of the points in $\mathcal{O}_b(x, S)$ from LiDAR to the ground and denote the set of the oblique projections as $\mathcal{O}^p(x, S).$ These projections are calculated via similar triangles. The occupied area $\mathcal{U}$ is computed as the convex hull of the union of $\mathcal{P}(\mathcal{O}_b(x, S))$ and $\mathcal{O}^p(x, S)$. The convex hull can be calculated via open-source tools such as Scipy~\cite{virtanen2020scipy}.

\begin{lemma}
    Given the observation of an obstacle $\mathcal{O}_b(x,S)$ and the the set of the oblique projections $\mathcal{O}^p(x, S).$ If occupied area $\mathcal{U}$ is computed as the convex hull of the union of $\mathcal{P}(\mathcal{O}_b(x, S))$ and $\mathcal{O}^p(x, S)$, then the vertical projections of the points of the obstacle are in $\mathcal{U}$.
\end{lemma}

\begin{proof}
    Suppose there is a point $p = (s^r, s^a, s^{\phi})$ of the obstacle. Without loss of generality, we set $s^a = a$ and $s^{\phi} = \phi$. We consider two cases, namely (i) there is line-of-sight between the LiDAR and $p$, and (ii) there is no line-of-sight between the LiDAR and $p.$

    \textit{Case (i):} In this case, $p \in \mathcal{O}_b(x,S).$ The vertical projection $\mathcal{P}(p) \in \mathcal{P}(\mathcal{O}_b(x, S)),$ and will be included in the convex hull of the union of $\mathcal{P}(\mathcal{O}_b(x, S))$ and $\mathcal{O}^p(x, S)$. Thus, $\mathcal{P}(p) \in \mathcal{U}.$

    \textit{Case (ii):} In this case, $p \notin \mathcal{O}_b(x,S).$ There exists at least one point $p^{\prime}$ in $\mathcal{O}_b(x,S)$ 
\end{proof}

\subsection{Augmented Perception}
The intuition is to utilize redundant information contained in the LiDAR observations of other agents. To do so, we introduce augmented perception. %Given a fixed Cartesian coordinate with origin $O_c$. 
For each agent indexed, we augment its perception by merging LiDAR observations of other agents $j\in L$. Specifically, we have the augmented scan represented as $S_i \oplus\boldsymbol{S}$, where $\boldsymbol{S}:=\{\bigcup_{j\neq i,j\in L}S^i_j\})$ and the augmented observation $\Tilde{\mathcal{O}}_i(x_i, S_i \oplus\boldsymbol{S})$ centered at $x_i$, where $S^i_j$ is the translated scan $S_j$ under Agent $i$'s coordinate.

Suppose there exists an Agent A with scan $S_A$ and occupied area $\mathcal{U}_A.$ The nearby Agent B provides its scan $S_B$ and occupied area $\mathcal{U}_B$ to Agent A. 
We define the augmented perceptions centered at $\mathbf{x}_A$ in $\mathcal{U}_A \cup \mathcal{U}_B$ as $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A)$ and $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_B)$. We calculate $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A)$ and $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_B)$ as follows.
\begin{align}
    &\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A) = \{\underbrace{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)}_{\Tilde{\mathcal{O}}_1}  \nonumber\\
    \label{eq:augmented-perception-A}
    &\cup \underbrace{(\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \setminus \mathcal{U}_B)}_{\Tilde{\mathcal{O}}_2} \cup \underbrace{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)}_{\Tilde{\mathcal{O}}_3}\}
    % &\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_B) = \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup (\mathcal{P}(\mathcal{O}_b(x_A, S_B)) \setminus \mathcal{U}_A) \nonumber\\
    % \label{eq:augmented-perception-B}
    % &\cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
\end{align}

\begin{table}[]
    \centering
    \begin{tabular}{ |c|c| } 
     \hline
     Attack & $(\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \setminus \mathcal{U}_B)$\\ 
     \hline
     true obstacle & $\emptyset$ \\
     a & $(\mathcal{P}(\mathcal{O}_b(x_A, S_A))$   \\ 
     b1 & $(\mathcal{P}(\mathcal{O}_b(x_A, S_A))$  \\ 
     b2 & $(\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \setminus \mathcal{U}_B)$  \\
     b3 & $\emptyset$  \\
     c & $\emptyset$  \\
     \hline
    \end{tabular}
    \caption{Impacts of Attacks on Observations and Occupied Areas}
    \label{tab:impacts-of-attacks}
\end{table}

Both $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A)$ and $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_B)$ consist of 3 parts. We use $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A)$ as an example to illustrate the 3 parts. $\Tilde{\mathcal{O}}_1$ corresponds to the projections of the observation that are observed by Agent A only. $\Tilde{\mathcal{O}}_2$ presents the projections of the obstacle observation of Agent A that does not belong to the occupied area of Agent B. %$\Tilde{\mathcal{O}}_3$ is the projections of the obstacle observation of Agent B that does not belong to the occupied area of Agent A. 
$\Tilde{\mathcal{O}}_3$ is the projections of the observation that are observed by Agent B only. 

% We propose Algorithm \ref{alg:AugPerception} to collect the augmented perceptions of Agent A and B centered at $\mathbf{x}_A$. 

% \begin{algorithm}[!htbp]
% \caption{Augmented Perceptions Centered at $\mathbf{x}_A$}
% \begin{algorithmic}[1]
%     \State \textbf{Input:} system states $\mathbf{x}_A$ and $\mathbf{x}_B$, observations $\mathcal{O}_A(\mathbf{x}_A, S_A)$ and $\mathcal{O}_B(\mathbf{x}_A, S_B)$
%     \State \textbf{Output:} augmented observations $\Tilde{\mathcal{O}}(\mathbf{x}_A, S_A)$ and $\Tilde{\mathcal{O}}(\mathbf{x}_A, S_B)$
%     % \For{$i \in L$}
%         % \State Set relative pose $r^{\prime}\gets O_c-\hat{x}_i$
%         % \State $p_i\gets p_i+r^{\prime}$, $\forall p_i \in \Tilde{\mathcal{O}}_i(x_i,S_i)$ denoted as $\Tilde{\mathcal{O}}_i(O_c,S_i) $
%         \For{$j\neq A, j\in L$}
%             \For{$\mathcal{P}_k\in(\mathcal{I}_j \cap \mathcal{U}_i)$}
%             % \State Transfer point $\Tilde{p}_k \gets  p_k + \hat{x}_i-\hat{x}_j$
%             % \State Transfer point $\Tilde{p}_k \in S^i_j$ from $p_k in S_j$  
%             \State $\Tilde{S}_i \gets S_i \cup \Tilde{p}_k$
%             \State Augment perception $\Tilde{\mathcal{O}}_i(x_i,\Tilde{S}_i)$
%             \EndFor
%         \EndFor
%     % \EndFor
% \end{algorithmic}
% \label{alg:AugPerception}
% \end{algorithm}


\subsection{Scan Match}
We assume that the NDT method subdivides the surrounding space uniformly into cells small enough so that each cell will contain at most one point of the observation. In this case, if a cell contains the point $q^{\prime},$ then the corresponding normal distribution will have mean $q = q^{\prime}.$ Thus, the scan match of the same observation $\mathcal{O}(\mathbf{x}_1, S_1)$ is $n_s,$ which means $r = 0$ and $\mathcal{L}_s(r) = n_s$.


\subsection{Impact of Attacks}
Since different attacks have different abilities and purposes, the impacts of the attacks on the observations and occupied areas are also different. %We conclude the impacts in the following table for later analysis. 
% \begin{table}[]
%     \centering
%     \begin{tabular}{ |c|c|c|c|c|c|c| } 
%      \hline
%      Attack & $\mathcal{O}(x_A, S_A)$ & $\mathcal{O}_b(x_A, S_A)$ & $\mathcal{U}_A$ & $\mathcal{O}(x_A, S_B)$ & $\mathcal{O}_b(x_A, S_B)$ & $\mathcal{U}_B$\\ 
%      \hline
%      a & move & up & up & - & - & -  \\ 
%      b1 & move & move & up & - & - & - \\ 
%      b2 & move & move & up & - & - & - \\
%      b3 & move & move & up & - & - & - \\
%      c & unch & unch & unch & unch & unch & unch \\
%      \hline
%     \end{tabular}
%     \caption{Impacts of Attacks on Observations and Occupied Areas}
%     \label{tab:impacts-of-attacks}
% \end{table}

For Attack a, the points of observation $\mathcal{O}(x_A, S_A)$ of the compromised LiDAR are changed, which introduces $\mathcal{O}_b(x_A, S_A)$ and corresponding $\mathcal{U}_A$. For Attack b1, b2, and b3, the $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}_b(x_A, S_A)$ corresponding to the original obstacle are changed to fail the LiDAR detection algorithm. In order to achieve that, $\mathcal{U}_A$ has to be enlarged to fully cover the original obstacle. For Attack c, $\mathcal{O}(x, S)$, $\mathcal{O}_b(x, S)$, and $\mathcal{U}$ are unchanged for all compromised LiDAR sensors.

% \begin{table}[]
%     \centering
%     \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%      \hline
%      Attack & $\mathcal{P}(\mathcal{O}(x_A, S_A))$ & $\mathcal{P}(\mathcal{O}_b(x_A, S_A))$ & $\mathcal{U}_A$ & $\Tilde{\mathcal{O}}_1$ & $\Tilde{\mathcal{O}}_2$ & $\Tilde{\mathcal{O}}_3$ & $\Tilde{\mathcal{O}}_4$\\ 
%      \hline
%      a & move & up & up & unch & up & unch & up \\ 
%      b1 & move & move & up & down & up & down & up \\ 
%      b2 & move & move & up & down & change & down & up \\
%      b3 & move & move & up & down & down & down & up \\
%      c & unch & unch & unch & unch & unch & unch & unch \\
%      \hline
%     \end{tabular}
%     \caption{Decision Table}
%     \label{tab:my_label}
% \end{table}
 


\subsection{Fault Detection, Identification, and Isolation}
\label{sec:FDII}
The objective of the proposed fault detection, identification, and isolation (FDII) algorithm is to detect the mismatch between the augmented observations of different agents, identify the spoofed agent, isolate the corrupted parts of the raw data, and restore the true unsafe region. The proposed FDII algorithm is illustrated as Fig.~\ref{fig:FDII}.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figs/decision_tree.png}
    \caption{Decision tree of the FDII algorithm.}
    \label{fig:FDII}
\end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{ |c|c|c|c| } 
     \hline
     Type of Attack & detect i & $U_i$ Non-Empty & Scan Match \\ 
     \hline
     None True & T & T & T \\ 
     None False & F & F & - \\ 
     a & T & T & F \\ 
     b1, b2 & F & T & F \\ 
     b3, c & F & T & T \\
     \hline
    \end{tabular}
    \caption{Decision Table}
    \label{tab:my_label}
\end{table}

The intuition is that if the LiDAR observation of an agent is spoofed by the adversary, the measured point $e^{\prime}$ in spoofed area $\varepsilon$ will not match the data collected by other agent $b\neq a$, $b\in L$. We limit the scope of scan match of the observation to the union of the occupied areas $\mathcal{U}_a\cup \mathcal{U}_b$ of two augmented observation $\Tilde{\mathcal{O}}_a^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_b^{\mathcal{I}}$. 
We also limit the scope of scan match of the observation to the horizontal axes of two augmented observations $\Tilde{\mathcal{O}}_a^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_b^{\mathcal{I}}$. 
% If it is a 2-D LiDAR, we use $\Tilde{\mathcal{O}}_i^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_j^{\mathcal{I}}$. If it is a 3-D LiDAR, we use the values of x and y coordinates of $\Tilde{\mathcal{O}}_i^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_j^{\mathcal{I}}$, which means the projection of the scan on the horizontal plane. 

The following lemma guarantees the detection of the mismatch between observations even if the spoofer presents.

\begin{lemma}
Suppose the object detection algorithms of Agent A outputs the bounding boxes $\mathcal{B}_A$ and the obstacle set $\mathcal{O}_b(x_A, S_A)$ inside $\mathcal{B}_A$. Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied areas $\mathcal{U}_A$ and $\mathcal{U}_B$ of Agent A and Agent B, respectively, and the obstacle set $\mathcal{O}_b(x_A, S_B)$ which has $\mathcal{P}(\mathcal{O}_b(x_A, S_B)) \subseteq \mathcal{U}_A$. If $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then either there exists a true obstacle in $\mathcal{B}_A$ or Attack b3/c occurs. Otherwise, Agent A is under Attack a or Attack b1/b2. 
\end{lemma}

\begin{proof}
    We first show that if neither there exists a true obstacle in $\mathcal{B}_A$ nor Attack b3/c occurs, which means either Attack a or Attack b1/b2 occur, then $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \neq n_s$. We consider two cases, namely (i) there exists a falsified obstacle and (ii) there exists Attack b1 or Attack b2 which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$.

    \textit{Case (i):} In this case, Agent A is under Attack a and we have $\mathcal{U}_A \neq \emptyset$ and $\mathcal{U}_B = \emptyset.$ Since there is only one attack, Agent B is attack-free and $\mathcal{O}_b(x_A, S_B) = \emptyset.$ According to Eq.~\eqref{eq:augmented-perception-A} and~\eqref{eq:augmented-perception-B}, the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
\begin{align*}
    \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \\
    &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
    =& \{\mathcal{P}(\mathcal{O}_b(x_A, S_A))\cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
    \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_B))\\
    &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}\\
    =&\{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}
\end{align*}

    Since $\Tilde{\mathcal{O}}(x_A, S_A) \neq \Tilde{\mathcal{O}}(x_A, S_B),$ the extra term $\mathcal{P}(\mathcal{O}_b(x_A, S_A))$ in $\Tilde{\mathcal{O}}(x_A, S_A)$ will introduce difference in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$

    \textit{Case (ii):} In this case, $\mathcal{P}(\mathcal{O}_b(x_A, S_B)) \subseteq \mathcal{U}_A$. However, $\mathcal{P}(\mathcal{O}_b(x_A, S_A))$ is not a subset of $\mathcal{U}_B$, which means that there exist elements in $\mathcal{P}(\mathcal{O}_b(x_A, S_A))$ that is also elements in $\mathcal{I}_B \setminus \mathcal{U}_B$. The augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follows.
\begin{align*}
    \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \\
    &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
    \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_B))\\
    &\cup (\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \cap \mathcal{U}_B ) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
\end{align*}

    Since there exist elements in $\mathcal{P}(\mathcal{O}_b(x_A, S_A))$ that is not in $\mathcal{U}_B$, we have $(\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \cap \mathcal{U}_B) \subseteq \mathcal{P}(\mathcal{O}_b(x_A, S_A))$ and there are more points in $\Tilde{\mathcal{O}}(x_A, S_A)$ than in $\Tilde{\mathcal{O}}(x_A, S_B)$. This will introduce differences in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$

    In both Case (i) and Case (ii), we have $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \neq n_s$, which proves that if neither there exists a true obstacle in $\mathcal{B}_A$ nor Attack b3/c occurs, then $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \neq n_s$. Hence, the converse-negative proposition that 'if $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then either there exists a true obstacle in $\mathcal{B}_A$ or Attack b3/c occurs' holds as well.

    Next, we show that if neither Attack 1 nor Attack b1/b2 occurs, which means that either there exists a true obstacle in $\mathcal{B}_A$ or Attack b3/c occurs, then $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$. In both cases, according to Eq.~\eqref{eq:augmented-perception-A} and~\eqref{eq:augmented-perception-B}, the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
    \begin{align*}
    \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \\
    &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
    \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_B))\\
    &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
    \end{align*}

    Since $\Tilde{\mathcal{O}}(x_A, S_A) = \Tilde{\mathcal{O}}(x_A, S_B),$ we have $r = 0$ and $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, which proves that if neither Attack 1 nor Attack b1/b2 occurs, then $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$. Hence, the converse-negative proposition that 'if $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \neq n_s$, then either Attack 1 or Attack b1/b2 occurs' holds as well.
\end{proof}

% \begin{lemma}
% Suppose the object detection algorithms of Agent A outputs the bounding boxes $\mathcal{B}_A$ and the obstacle set $\mathcal{O}_b(x_A, S_A)$ inside $\mathcal{B}_A$. Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied areas $\mathcal{U}_A$ and $\mathcal{U}_B$ of Agent A and Agent B, respectively, and the obstacle set $\mathcal{O}_b(x_A, S_B)$ which has $\mathcal{P}(\mathcal{O}_b(x_A, S_B)) \subseteq \mathcal{U}_A$. If $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then there exists a true obstacle in $\mathcal{B}_A$. Otherwise, Agent A is under Attack a. 
% % Suppose the object detection algorithms of Agent A outputs the bounding boxes $\mathcal{B}_A$. Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied area $\mathcal{U}_A$ and $\mathcal{U}_B,$ the sets of projection of the points inside $\mathcal{B}_A$ on the horizontal plane $O_A,$ and the set of projection of $O_B$, If the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ match, then there exists a true obstacle
% % Suppose the object detection algorithms of Agent A and B output the bounding boxes $\mathcal{B}_A$ and $\mathcal{B}_B$ for the same obstacle, respectively. Given the sets of projection of the points inside $\mathcal{B}_A$ and $\mathcal{B}_B$ on the horizontal plane $O_A$ and $O_B$, the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, and the occupied area $\mathcal{U}_A$ and $\mathcal{U}_B.$ If the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ match, then there exists a true obstacle

% \end{lemma}

% \begin{proof}
% We consider two cases, namely (i) there exists a true obstacle in $\mathcal{B}_A$ and (ii) there exists a falsified obstacle.

% \textit{Case (i):} In this case, the spoofer does not present. We calculate the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate as follow.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_B))\\
%     &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
% \end{align*}

% Since $\Tilde{\mathcal{O}}(x_A, S_A) = \Tilde{\mathcal{O}}(x_A, S_B),$ we have $r = 0$ and $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s.$

% \textit{Case (ii):} In this case, Agent A is under Attack a and we have $\mathcal{U}_A \neq \emptyset$ and $\mathcal{U}_B = \emptyset.$ Since there is only one attack, Agent B is attack-free and $\mathcal{O}_b(x_A, S_B) = \emptyset.$ The augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     =& \{\mathcal{P}(\mathcal{O}_b(x_A, S_A))\cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_B))\\
%     &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}\\
%     =&\{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}
% \end{align*}

% Since $\Tilde{\mathcal{O}}(x_A, S_A) \neq \Tilde{\mathcal{O}}(x_A, S_B),$ the extra term $\mathcal{P}(\mathcal{O}_b(x_A, S_A))$ in $\Tilde{\mathcal{O}}(x_A, S_A)$ will introduce difference in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$

% % \textit{Case (i):} In this case, the spoofer does not present. We calculate the scan match $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B)$ as follow.
% % \begin{align*}
% %     &\quad\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \\
% %     &= \{((\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_\mathcal{B}(x_A, S_A)) \\
% %     &\quad\cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A))\}\\ 
% %     &\ominus ((Ground_B\cap U_A)\cup O_B\cup (e^{\prime}\cup Ground_A\cap U_B))
% % \end{align*}
% \end{proof}


% \begin{lemma}
% Suppose there exists the obstacle set $\mathcal{O}_b(x_A, S_A)$ with the occupied area $\mathcal{U}_A$, and the object detection algorithms of Agent A does not detect any obstacle with vertical projection in $\mathcal{U}_A$.
% Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied areas $\mathcal{U}_A$ and $\mathcal{U}_B$ of Agent A and Agent B, respectively, and the obstacle set $\mathcal{O}_b(x_A, S_B)$ which has $\mathcal{P}(\mathcal{O}_b(x_A, S_B)) \subseteq \mathcal{U}_A$. If $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then there exists Attack b3 or Attack c which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$. Otherwise, there exists Attack b1 or Attack b2 which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$. 
% \end{lemma}

% \begin{proof}
% We consider two cases, namely (i) there exists Attack b3 or Attack c which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$, and (ii) there exists Attack b1 or Attack b2 which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$.

% \textit{Case (i):} In this case, $\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \subseteq \mathcal{U}_B$ and $\mathcal{P}(\mathcal{O}_b(x_A, S_B)) \subseteq \mathcal{U}_A$. We calculate the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate as follow.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_B))\\
%     &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
% \end{align*}

% Since $\Tilde{\mathcal{O}}(x_A, S_A) = \Tilde{\mathcal{O}}(x_A, S_B),$ we have $r = 0$ and $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s.$

% \textit{Case (ii):} In this case, $\mathcal{P}(\mathcal{O}_b(x_A, S_B)) \subseteq \mathcal{U}_A$. However, $\mathcal{P}(\mathcal{O}_b(x_A, S_A))$ is not a subset of $\mathcal{U}_B$, which means that there exist elements in $\mathcal{P}(\mathcal{O}_b(x_A, S_A))$ that is also elements in $\mathcal{I}_B \setminus \mathcal{U}_B$. The augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}_b(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}_b(x_A, S_B))\\
%     &\cup (\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \cap \mathcal{U}_B ) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
% \end{align*}

% Since there exist elements in $\mathcal{P}(\mathcal{O}_b(x_A, S_A))$ that is not in $\mathcal{U}_B$, we have $(\mathcal{P}(\mathcal{O}_b(x_A, S_A)) \cap \mathcal{U}_B) \subseteq \mathcal{P}(\mathcal{O}_b(x_A, S_A))$ and there are more points in $\Tilde{\mathcal{O}}(x_A, S_A)$ than in $\Tilde{\mathcal{O}}(x_A, S_B)$. This will introduce difference in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$
% \end{proof}


We consider three LiDAR attacks presented in Sec.~\ref{subsec:threat-model} as shown in Fig.~\ref{fig:three-LiDAR-attacks}. Without loss of generality, we show the idea by using two agents.

The following lemma shows that the unsafe region can be achieved even if the three LiDAR attacks occur.

\begin{lemma}
    decision tree
\end{lemma}

Based on the results of Lemma ..., we propose the function ... in Algorithm~... to generate unsafe regions that can be used to provide feasible control inputs to guarantee safety requirements.

The rules to update unsafe regions based on multi-agent observations.
\begin{enumerate}
    \item If an occupied area is only observed by one agent, then it covers a falsified non-existing obstacle resulted from a relay attack.

    \item If an occupied area 
\end{enumerate}

Only consider the intersection of occupied area when doing mismatch detection.
\begin{enumerate}
    \item For attack a and b1 (non-existing obstacle), the intersection is empty.

    \item For attack b2 (Agent j could partically observe the area covered by Agent i's occupied area), we could narrow the range of the intersection based on the observation of Agent j.

    \item For attack b3 and c (Agent j cannot observe the area covered by Agent i's occupied area), we append the intersection into the updated unsafe region.
\end{enumerate}

Challenges:
\begin{enumerate}
    \item How to identify the occupied area?

    Divide the overlapping area of the observations $\Tilde{\mathcal{O}}_i(O_c,S_i)$ and $\Tilde{\mathcal{O}}_j(O_c,S_j)$ uniformly into small cells with constant size. If there is no point $p_i$ inside the cell, we consider the empty cell as a part of an occupied area of Agent $i$. The nearby empty cells combine together as an occupied area. The adjacent nonempty cells are considered as the boundary of the occupied area.

    \item How to do augmented perception?

    Do not need augmented perception in this case.

    \item How to do mismatch detection?

    Do not need to do mismatch detection in this case. 
\end{enumerate}

In Fig.~\ref{fig:RelayExp}, the spoofer falsifies a non-existing obstacle in the raw data of the attacked Agent $i$ by firing laser beams to the receiver of the LiDAR. The augment perception $\Tilde{\mathcal{O}}_i(O_c,\Tilde{S}_i)$ of Agent $i$ is obtained by combining points $\Tilde{p}_k$ in the overlapping area of the falsified occupied area $\mathcal{U}_i$ and the scan covered area $\mathcal{I}_j$. This overlapping area is guaranteed to exist and be the same as $\mathcal{U}_i$ by Eq.~\eqref{eq:jointpercept}. The augment perception $\Tilde{\mathcal{O}}_j(O_c,\Tilde{S}_j)$ of Agent $j$ is identical with the observation $\Tilde{\mathcal{O}}_j(O_c,S_j)$ because there is no occupied area in the raw data. Thus, there is mismatch of the observation in the overlapping area $\mathcal{I}_i\cap \mathcal{I}_j$ of two augmented observation $\Tilde{\mathcal{O}}_i^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_j^{\mathcal{I}}$.

In Fig.~\ref{fig:PRAExp}, the spoofer implements PRA by creating a falsified obstacle between Agent $i$ and the true obstacle. Since the position of the falsified obstacle and the position of the true obstacle are different, there exists occupied area that can only be detected by one of the agent, which means $\mathcal{U}_i \neq \mathcal{U}_j$. According to Eq.~\eqref{eq:jointpercept}, $\mathcal{U}_i \subseteq \mathcal{I}_j$ and $\mathcal{U}_j \subseteq \mathcal{I}_i.$ Thus, $(\mathcal{I}_j \cap \mathcal{U}_i) = \mathcal{U}_i \neq \mathcal{U}_j = (\mathcal{I}_i \cap \mathcal{U}_j)$.

In Fig.~\ref{fig:AdvObjExp}, 

We compute relative pose by performing scan match $\Tilde{\mathcal{O}}_i^{\mathcal{I}} \ominus \Tilde{\mathcal{O}}_j^{\mathcal{I}}$. 

\begin{proposition}
    (Working on *proposition)
\end{proposition}
If the relative pose exceed a threshold derived by (*proposition), it means one of the scans is spoofed. We next identify the area affected spoofed data by solving the following optimization problem  
\begin{equation}
    \label{eq:FIdent}
    \min_c (\Tilde{\mathcal{O}}_i^{\mathcal{I}} \backslash c)\ominus (\Tilde{\mathcal{O}}_j^{\mathcal{I}} \backslash c)
\end{equation}
With the mismatched area spotted, we then formulate decision tree to identify the attack type and spoofed agent. 

(working on) train of thought: We summarize the symptom of different attack type and formulate the Decision tree 



We finally proposed Alg. \ref{alg:FDII} to summarize the workflow. 
% \begin{algorithm}[!htbp]
% \caption{LiDAR Fault Detection, Identification and Isolation}
% \begin{algorithmic}[1]
%     \State \textbf{Input:} A set of augmented LiDAR Observation $\boldsymbol{\Tilde{\mathcal{O}}}:=\{\Tilde{\mathcal{O}},\forall i\in L\}$
%     \State \textbf{Output:} 
%     \For{$i,j\in L$}
%         \State Compute $r \gets \Tilde{\mathcal{O}}_i^{\mathcal{I}} \ominus \Tilde{\mathcal{O}}_j^{\mathcal{I}}$
%         \If{$r>\theta$}
%             \State Solve \eqref{eq:FIdent}
%             \State (Working on)
%         \EndIf
%     \EndFor
% \end{algorithmic}
% \label{alg:FDII}
% \end{algorithm}


% \subsection{Safety Region Estimation}
\subsection{Safe Control}
% \input{sections/control.tex}
\input{sections/control_v1.tex}
% We next design a safe control methodology to ensure safety of the controlled agent with desired probability. We formulate it as a control of a hybrid system. 

% In section \ref{sec:FDII}, we detect and estimate the obstacle to acquire unsafe region $h_1(x)$. Hence, we have the safe set as $\mathcal{C}_1:=\{x\mid h_1(x)\geq0\}$. 

==> sections/ProposedMethod_v2.tex <==
\section{Proposed Detection and Control Approach}
\label{sec:methodology}
In this section, we propose a detection and control approach to keep the safety of the vehicle under an adversarial environment. The proposed approach is illustrated as Fig.~\ref{fig:illustration}. The vehicle collects environmental perception from the neighboring vehicles, detects the attacks and updates the unsafe region based on the environmental perception, and executes safe control signal based on the updated unsafe region.
% In this section, we propose a fault-tolerant augmented perception to obtain an accurate environmental estimation. The proposed approach is illustrated as Fig.~\ref{fig:illustration}. At each time, Agent A collects the current observations of nearby agents $\mathcal{O}(x_j, S_j), \forall j \in L, j \neq A$ and calculates necessary information. Then the occupied areas are computed based on $\mathcal{O}(x_j, S_j), \forall j \in L$. Next, the FDII module detects and classifies the attacks, and updates the unsafe region based on the occupied areas.

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figs/illustration.png}
    \caption{Schematic illustration of the proposed approach.}
    \label{fig:illustration}
\end{figure}

\subsection{Occupied Area Identification}
\label{subsec:occupied-area-identification}
In this subsection, we present our method to identify and extract the area that either contains obstacles or is not observable by the LiDAR, which we denote the occupied area. The detected occupied area will then be combined with the information from other vehicles to detect attacks and compute the unsafe region (Section~\ref{sec:FDII}).

We first prune the raw data of the observation $\mathcal{O}(x, S)$ by removing the points corresponding to the infrastructure (for example, walls) on a default map. For the rest of the paper, we use $\mathcal{O}(x, S)$ to denote the pruned observation. %The remaining points 
We define the scan-covered area $\mathcal{I}_j = \mathcal{P}(\mathcal{O}(x, S))$ under $\mathcal{O}^b_k(x, S) = \emptyset$ as the projection of the observation of Agent $j$ if there is no obstacle. 
% Define $r_j$ as the maximum range that can be observed by Agent $j$. We define the scan-covered area $\mathcal{I}_j = \mathcal{P}(\mathcal{O}(x, S)), \mathcal{O}^b_k(x, S) = \emptyset$ as the area on the default map that can be observed by the Agent $j$ if there is no obstacle. 
% Let the true observed area of the observation be denoted as $\mathcal{I} = \mathcal{P}(\mathcal{O}(x, S))$. 
For Agent A, denote $L:= \{j: \mathcal{I}_A \cap \mathcal{I}_j \neq \emptyset\}$ as the set of agents which have an overlapping scan-covered area with Agent A. 
We define the vertical projection operation $\mathcal{P}(\mathcal{O}(x, S))\longrightarrow \mathcal{Y},$ which takes an observation $\mathcal{O}(x, S)$ as input and outputs the set $\mathcal{Y}$ of the projections of the points in $\mathcal{O}(x, S)$ onto the $x\text{-}y$ coordinate plane. %Denote the set of points corresponding to the obstacles as $\mathcal{O}^b_k(x,S) := \{p=(o^x, o^y, o^z), o^z > \zeta^z\}$. 

We utilize the altitude coordinates of the points to distinguish the ground and the obstacle as described in~\cite{qian2014ncc}\cite{bogoslavskyi2017efficient}. We let $\zeta^z$ denote the estimation error of the altitude coordinate.
The detection algorithm identifies $p_i = (o_i^x, o_i^y, o_i^z)$ as belonging to the ground if $o_i^z \leq \zeta^z$ and belonging to an obstacle if $o_i^z > \zeta^z.$
% For point $p_i = (o^x_i, o^y_i, o^z_i)$ in $\mathcal{O}(x, S),$ $\forall i \in n_s,$ if $o^z_i \leq \zeta^z,$ where $\zeta^z$ is the estimation error of the altitude coordinate, then $p_i$ belongs to the ground. If $o^z_i > \zeta^z,$ then $p_i$ is part of an obstacle. This scheme has been used to remove the ground from 3D scans~\cite{qian2014ncc}\cite{bogoslavskyi2017efficient}.

After ground removal, we use the 3D bounding box provided by the LiDAR-based 3D object detection algorithms of the autonomous vehicles (AVs)~\cite{zamanakos2021comprehensive} to cluster the points into a collection of obstacles, denoted $O_k^b(x,S) \subseteq O(x,S).$ Here, the index $k$ ranges from $1$ to $n_o^j,$ where $n_o^j$ denotes the number of obstacles detected by Agent $j$. Note that the set $O_1^b(x,S),\ldots,O_{n_o^j}^b(x,S)$ may contain fake obstacles introduced by an adversary.
% After ground removal, we obtain points corresponding to the observations of the obstacles $\mathcal{O}^b_k(x,S) := \{p=(o^x, o^y, o^z)\textcolor{blue}{:} o^z > \zeta^z\}$, where $k \in \{1,\ldots,n^j_o\}$ is the index of the obstacles (including any non-existing obstacles introduced by Attack NEO) observed by Agent $j$ and $n^j_o$ is the number of the obstacles observed by Agent $j.$ To determine the boundaries of the observations $\mathcal{O}^b_k(x,S)$, we use the 3D bounding box provided by the LiDAR-based 3D object detection algorithms of the autonomous vehicles~\cite{zamanakos2021comprehensive}. The bounding box describes the location, size, and orientation of an object in 3D space. We consider the points that belong to one bounding box as the observation of one obstacle. 
\textcolor{red}{We regard the points that do not belong to any bounding box as the points introduced by Attack PRA or Attack AO. }
% Since there is at most one \textcolor{blue}{Attack PRA} or \textcolor{blue}{Attack AO} which hides the object from the object detection algorithms, we regard the points that do not belong to any bounding box as the points of one obstacle. %Denote the average of the points in $\mathcal{O}^o(x, S)$ as $\Bar{o}$, and the maximum distance between the points in $\mathcal{O}^o(x, S)$ and $\Bar{o}$ as $d = \max \|\|$
We further calculate the oblique projections $\mathcal{O}^p_k(x, S)$ of the points in $\mathcal{O}^b_k(x, S)$, which consists of the points where a straight line from the sensor to each point in $\mathcal{O}^b_k(x, S)$ intersects the ground.
% We further calculate the oblique projections $\mathcal{O}^p_k(x, S)$ of the points in $\mathcal{O}^b_k(x, S)$ as follows. Suppose $p \in \mathcal{O}^b_k(x, S).$ We draw a line from the LiDAR to $p$. The line intersects the ground at point $p_g$, which is regarded as the element of $\mathcal{O}^p_k(x, S).$
% We further calculate the oblique projections of the points in $\mathcal{O}^b_k(x, S)$ from LiDAR to the ground and denote the set of the oblique projections as $\mathcal{O}^p(x, S).$ The points in $\mathcal{O}^p(x, S)$ are calculated as follows. Suppose $p \in \mathcal{O}^b_k(x, S).$ We draw a line between $p$ and the LiDAR, and choose the point on the line with $o^z = 0$ as the element of $\mathcal{O}^p(x, S).$ %These projections are calculated via similar triangles. 



We let $\mathcal{U}_{jk}$ denote the occupied area corresponding to Obstacle $k$ observed by Agent $j$, which consists of the area that contains the obstacle as well as the area that is obscured by the obstacle.
The occupied area $\mathcal{U}_{jk}$ is computed as the convex hull of $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$. The convex hull can be calculated via open-source tools such as Scipy~\cite{virtanen2020scipy}. 
In order to compute the convex hull, we first obtain a collection of pairs of points $\{(x_1^l,y_1^l), (x_2^l, y_2^l): l=1,\ldots,n_{jk}^h\}$ from the object detection and oblique projection algorithms, where $n_{jk}^h$ is the number of the boundaries of Obstacle $k$ observed by Agent $j$. For each pair indexed $l$, we compute a half-plane constraint $h^{jk}_l(x) \leq 0$ with $h^{jk}_l(x) =  a^{jk}_l \times x + b^{jk}_l$ where $a^{jk}_l$ and $b^{jk}_l$ are defined as $a^{jk}_l = \frac{y^l_2 - y^l_1}{x^l_2 - x^l_1}$ and $b^{jk}_l = \frac{x^l_2 \times y^l_1 - x^l_1 \times y^l_2}{x^l_2 - x^l_1}.$ The convex hull is equal to the intersection of the half-plane constraints, i.e., 
$$U_{jk} = \bigcap_{l=1}^{n_{jk}^h}{\{x : h_{l}^{jk}(x) \leq 0\}}.$$
% The convex hull contains all points in $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$ and the segments between those points. The boundaries $h^{jk}_l(x) =  a^{jk}_l \times x + b^{jk}_l = 0$ of the convex hull corresponding to the occupied area $\mathcal{U}_{jk}$ are a collection of line segments, where $l \in \{1,\ldots,n^h_{jk}\}$ is the number of the boundaries of obstacle $k$ observed by Agent $j$, $a^{jk}_l = \frac{y^l_2 - y^l_1}{x^l_2 - x^l_1}$, $b^{jk}_l = \frac{x^l_2 \times y^l_1 - x^l_1 \times y^l_2}{x^l_2 - x^l_1},$ and $(x^l_1, y^l_1),$ $(x^l_2, y^l_2)$ are the two vertices of the boundary. The vertices of the boundaries are the points in $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$. For $x$ that satisfies $h^{jk}_l(x) \leq 0, \forall l \in \{1,\ldots,n^h_{jk}\},$ it belongs to the convex hull. 
% The convex hull chooses some points in $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$ and uses the segments between those chosen points to surrounding all points in $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$ and the segments between all points. 
% The convex hull is calculated as the envelope lines that surround the points in $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$. The vertices of the envelope lines are the elements of $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$. 

The occupied area computed by the above procedure may not fully contain the obstacle due to the fact that the obstacle location must be interpolated from a finite number of samples. We enhance the robustness of these sampling errors by changing the boundaries of the convex hull to $h_l^{jk}(x) - \zeta_h \leq 0,$ where $\zeta_h = \zeta_n + \zeta_r$, where $\zeta_n$ is the observation noise bound and $\zeta_r$ is a bound on the distance between neighboring sample points that can be obtained from the distance to the object and the angular resolution of the LiDAR. \textcolor{red}{We assume that the LiDAR resolution is sufficiently large such that each point on the obstacle that is in the line-of-sight of the LiDAR is at most $\zeta_r$ distance away from at least one scan point.}
% Due to the limitation of the resolution of LiDAR, only a finite number of points on the obstacle can be scanned. The straight-line distance between the projections of two neighboring scanned points can be calculated based on the technical specification of the LiDAR. 
% % Due to the existence of the resolution of LiDAR, there are unscanned points on the obstacle, which are between two neighboring scan points (which belong to one obstacle, obstacle and ground, or two obstacles) and are not scanned by the LiDAR. The distance between two neighboring scan points can be calculated based on the horizontal and vertical resolutions and the ranges of the points. 
% Denote the straight-line distance between the projections of two neighboring scan points $p_i$ and $p_{i^{\prime}}$ as $d_{ii^{\prime}}.$ Denote the observation noise bound as $\zeta_n.$
% % We set the sum of the maximum of the distances between two neighboring scan points and the noise bound of the LiDAR observation as $\zeta_h.$ 
% % We set the sum of the maximum of the distances between two neighboring scan points and the noise bound of the LiDAR observation as $\zeta_h.$
% %If the projections of those unscanned points on the obstacle do not belong to the convex hull, we denote the distance of the unscanned points to the nearest boundary of the convex hull as $\zeta_h.$ 
% We enlarge the convex hull by changing the boundaries to $h^{jk}_l(x) - \zeta_h \leq 0,$ where $\zeta_h = \zeta_n + \max d_{ii^{\prime}}$.
% % We enlarge the convex hull by pushing each boundary of the convex hull along its normal direction to the outside by $\zeta_h = \zeta_n + \max d_{ii^{\prime}}$. 
% The enlarged convex hull contains the projection of the obstacle in a finite-resolution and noisy environment. %to account for the unscanned points on the obstacle that are between two neighboring scan points, the oblique projections of the unscanned points, and the observation noise. 
% % We enlarge the convex hull by extending each boundary of the convex hull along its normal direction by $\zeta_h$ to account for the unscanned points on the obstacle that are between two neighboring scan points, the oblique projections of the unscanned points, and the observation noise. 


At each time, Agent A collects the current observations of nearby agents $\mathcal{O}(x_j, S_j), \forall j \in L, j \neq A$. The corresponding observations $\mathcal{O}(x_A, S_j),$ the observations of obstacles $\mathcal{O}^b_k(x_A, S_j),$ and the occupied areas $\mathcal{U}_j$ are calculated by Agent A.

For each obstacle, define the set of points of the obstacle as $P^{ob}.$ For each agent, we divide the obstacle into two parts. The first part is the set of points in $P^{ob}$ that have line-of-sight with the LiDAR. We denote the first part as $P_1.$ The second part, which is denoted as $P_2,$ is the set of points in $P^{ob}$ that do not have line-of-sight with the LiDAR.

\begin{lemma}
\label{lemma:occupied-area-covers-obstacle-projection}
    Suppose we are given the observation of an obstacle $\mathcal{O}^b_k(x,S)$ in a bounding box and the set of oblique projections $\mathcal{O}^p(x, S).$ If occupied area $\mathcal{U}$ is computed as the convex hull of $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$, then $\mathcal{P}(P^{ob}) \subseteq \mathcal{U}.$%then the vertical projections of the points of the obstacle are in $\mathcal{U}$.
\end{lemma}

\begin{proof}
    As described above, $P^{ob} = P_1 \cup P_2.$ In what follows, we describe how $P_1 \subseteq \mathcal{U}$ and $P_2 \subseteq \mathcal{U},$ and hence $\mathcal{P}(P^{ob}) \subseteq \mathcal{U}.$
    % The obstacle $P^{ob}$ consists of two parts: the part $P_1$ that can be observed by a certain agent (eg. Agent A) with observation $\mathcal{O}^b_k(x, S),$ and the part $P_2$ that cannot be observed by Agent A (the interior and back side corresponding to Agent A's position).

    \underline{\textit{$P_1$}}: The points in $P_1$ either belong to $\mathcal{O}^b_k(x, S)$ or are between two neighboring scan points. For the points that belong to $\mathcal{O}^b_k(x, S)$, since the convex hull surrounds the points in $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$, the projections of the points that belong to $\mathcal{O}^b_k(x, S)$ are contained in the convex hull. 
    For the points that are between two neighboring scan points, since $\max_x h_l(x) \leq \zeta_h,$ they are contained in the convex hull $h_l(x) - \zeta_h \leq 0.$
    % For the points that are between two neighboring scan points, they are contained in the convex hull guaranteed by the margin $\zeta_h.$

    \underline{\textit{$P_2$}}: Suppose there is a point $p = (s^r, s^a, s^{\phi}) = (o^x, o^y, o^z) \in P_2.$ There must exist a point $p_{\ast} = (s^r_{\ast}, s^a_{\ast}, s^{\phi}_{\ast}) = (o^x_{\ast}, o^y_{\ast}, o^z_{\ast}) \in P_1$ such that $s^a = s^a_{\ast}$, $s^{\phi} = s^{\phi}_{\ast}$ and $s^r > s^r_{\ast},$ which block the line-of-sight between the LiDAR and $p.$ Since $s^a = s^a_{\ast}$ and $s^{\phi} = s^{\phi}_{\ast}$, the oblique projections of $p$ and $p_{\ast}$ are identical, which means that $p$, $p_{\ast}$, and $p_0$ are collinear.
    We denote the oblique projection of $p$ and $p_{\ast}$ as $p_o = (0, 0, 0)$ without loss of generality. 

    Next we would like to show that the projection $\mathcal{P}(p)$, the projection $\mathcal{P}(p_{\ast})$, and $p_0$ are collinear. 
    We have $\overrightarrow{p_0p} = (o^x, o^y, o^z)$ and $\overrightarrow{p_0p_{\ast}} = (o^x_{\ast}, o^y_{\ast}, o^z_{\ast})$. Since $p$, $p_{\ast}$, and $p_0$ are collinear, we have $\overrightarrow{p_0p} \times \overrightarrow{p_0p_{\ast}} = 0,$ which gives us
    \begin{align}
        \label{eq:collinear-obstacle-1}
        o^yo^z_{\ast} - o^zo^y_{\ast} &= 0 \\
        \label{eq:collinear-obstacle-2}
        o^zo^x_{\ast} - o^xo^z_{\ast} &= 0 \\
        \label{eq:collinear-obstacle-3}
        o^xo^y_{\ast} - o^yo^x_{\ast} &= 0 
    \end{align}
    Similarly, we have $\overrightarrow{p_0\mathcal{P}(p)} = (o^x, o^y, 0)$ and $\overrightarrow{p_0\mathcal{P}(p_{\ast})} = (o^x_{\ast}, o^y_{\ast}, 0)$. Then we can get $\overrightarrow{p_0\mathcal{P}(p)} \times \overrightarrow{p_0\mathcal{P}(p_{\ast})} = (0, 0, o^xo^y_{\ast} - o^yo^x_{\ast})$. According to Eq.~\eqref{eq:collinear-obstacle-3}, we have $\overrightarrow{p_0\mathcal{P}(p)} \times \overrightarrow{p_0\mathcal{P}(p_{\ast})} = (0, 0, 0),$ which means that the projection $\mathcal{P}(p)$, the projection $\mathcal{P}(p_{\ast})$, and $p_0$ are collinear.

    Finally, we would like to show that $\mathcal{P}(p)$ belongs to the convex hull. Since the convex hull contains $P_1$ and its oblique projection, $\mathcal{P}(p_{\ast})$ and $p_0$ belong to the convex hull. Since the convex hull is a convex set, it contains the line segment $\overline{p_0\mathcal{P}(p_{\ast})}.$ Since the projection $\mathcal{P}(p)$, the projection $\mathcal{P}(p_{\ast})$, and $p_0$ are collinear, $\mathcal{P}(p)$ belongs to the line segment $\overline{p_0\mathcal{P}(p_{\ast})},$ which means that $\mathcal{P}(p)$ belongs to the convex hull.

    Since both the projections of the points in $P_1$ and $P_2$ belong to the convex hull, and the occupied area $\mathcal{U}$ is computed as the convex hull of $\mathcal{P}(\mathcal{O}^b_k(x, S)) \cup \mathcal{O}^p(x, S)$, thus we have $\mathcal{P}(P^{ob}) \subseteq \mathcal{U}.$ 
    % \underline{\textit{$P_2$}}: Suppose there is a point $p = (s^r, s^a, s^{\phi}) = (o^x, o^y, o^z) \in P_2.$ There must exist a point $p_{\ast} = (s^r_{\ast}, s^a_{\ast}, s^{\phi}_{\ast}) = (o^x_{\ast}, o^y_{\ast}, o^z_{\ast}) \in P_1$ such that $s^a = s^a_{\ast}$,  and $s^{\phi} < s^{\phi}_{\ast}$
\end{proof}
% \begin{proof}
%     Suppose there is a point $p = (s^r, s^a, s^{\phi})$ of the obstacle. Without loss of generality, we set $s^a = a$ and $s^{\phi} = \phi$. We consider two cases, namely (i) there is a line-of-sight between the LiDAR and $p$, and (ii) there is no line-of-sight between the LiDAR and $p.$

%     \textit{Case (i):} In this case, $p \in \mathcal{O}^b_k(x,S).$ The vertical projection $\mathcal{P}(p) \in \mathcal{P}(\mathcal{O}^b_k(x, S)),$ and will be included in the convex hull of the union of $\mathcal{P}(\mathcal{O}^b_k(x, S))$ and $\mathcal{O}^p(x, S)$. Thus, $\mathcal{P}(p) \in \mathcal{U}.$

%     \textit{Case (ii):} In this case, $p \notin \mathcal{O}^b_k(x,S).$ There exists at least one point $p^{\prime}$ in $\mathcal{O}^b_k(x,S)$ 
% \end{proof}

% \subsection{Augmented Perception}
% The intuition is to utilize redundant information contained in the LiDAR observations of other agents. To do so, we introduce augmented perception. %Given a fixed Cartesian coordinate with origin $O_c$. 
% For each agent indexed, we augment its perception by merging LiDAR observations of other agents $j\in L$. Specifically, we have the augmented scan represented as $S_i \oplus\boldsymbol{S}$, where $\boldsymbol{S}:=\{\bigcup_{j\neq i,j\in L}S^i_j\})$ and the augmented observation $\Tilde{\mathcal{O}}_i(x_i, S_i \oplus\boldsymbol{S})$ centered at $x_i$, where $S^i_j$ is the translated scan $S_j$ under Agent $i$'s coordinate.

% Suppose there exists an Agent A with scan $S_A$ and occupied area $\mathcal{U}_A.$ The nearby Agent B provides its scan $S_B$ and occupied area $\mathcal{U}_B$ to Agent A. 
% We define the augmented perceptions centered at $\mathbf{x}_A$ in $\mathcal{U}_A \cup \mathcal{U}_B$ as $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A)$ and $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_B)$. We calculate $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A)$ and $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_B)$ as follows.
% \begin{align}
%     &\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A) = \{\underbrace{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)}_{\Tilde{\mathcal{O}}_1}  \nonumber\\
%     \label{eq:augmented-perception-A}
%     &\cup \underbrace{(\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B)}_{\Tilde{\mathcal{O}}_2} \cup \underbrace{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)}_{\Tilde{\mathcal{O}}_3}\}
%     % &\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_B) = \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup (\mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \setminus \mathcal{U}_A) \nonumber\\
%     % \label{eq:augmented-perception-B}
%     % &\cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
% \end{align}

% \begin{table}[]
%     \centering
%     \begin{tabular}{ |c|c| } 
%      \hline
%      Attack & $(\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B)$\\ 
%      \hline
%      true obstacle & $\emptyset$ \\
%      a & $(\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$   \\ 
%      b1 & $(\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$  \\ 
%      b2 & $(\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B)$  \\
%      b3 & $\emptyset$  \\
%      c & $\emptyset$  \\
%      \hline
%     \end{tabular}
%     \caption{Impacts of Attacks on Observations and Occupied Areas}
%     \label{tab:impacts-of-attacks}
% \end{table}

% Both $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A)$ and $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_B)$ consist of 3 parts. We use $\Tilde{\mathcal{O}}_{\mathcal{U}}^{AB}(x_A, S_A)$ as an example to illustrate the 3 parts. $\Tilde{\mathcal{O}}_1$ corresponds to the projections of the observation that are observed by Agent A only. $\Tilde{\mathcal{O}}_2$ presents the projections of the obstacle observation of Agent A that does not belong to the occupied area of Agent B. %$\Tilde{\mathcal{O}}_3$ is the projections of the obstacle observation of Agent B that does not belong to the occupied area of Agent A. 
% $\Tilde{\mathcal{O}}_3$ is the projections of the observation that are observed by Agent B only. 

% % We propose Algorithm \ref{alg:AugPerception} to collect the augmented perceptions of Agent A and B centered at $\mathbf{x}_A$. 

% % \begin{algorithm}[!htbp]
% % \caption{Augmented Perceptions Centered at $\mathbf{x}_A$}
% % \begin{algorithmic}[1]
% %     \State \textbf{Input:} system states $\mathbf{x}_A$ and $\mathbf{x}_B$, observations $\mathcal{O}_A(\mathbf{x}_A, S_A)$ and $\mathcal{O}^b_k(\mathbf{x}_A, S_B)$
% %     \State \textbf{Output:} augmented observations $\Tilde{\mathcal{O}}(\mathbf{x}_A, S_A)$ and $\Tilde{\mathcal{O}}(\mathbf{x}_A, S_B)$
% %     % \For{$i \in L$}
% %         % \State Set relative pose $r^{\prime}\gets O_c-\hat{x}_i$
% %         % \State $p_i\gets p_i+r^{\prime}$, $\forall p_i \in \Tilde{\mathcal{O}}_i(x_i,S_i)$ denoted as $\Tilde{\mathcal{O}}_i(O_c,S_i) $
% %         \For{$j\neq A, j\in L$}
% %             \For{$\mathcal{P}_k\in(\mathcal{I}_j \cap \mathcal{U}_i)$}
% %             % \State Transfer point $\Tilde{p}_k \gets  p_k + \hat{x}_i-\hat{x}_j$
% %             % \State Transfer point $\Tilde{p}_k \in S^i_j$ from $p_k in S_j$  
% %             \State $\Tilde{S}_i \gets S_i \cup \Tilde{p}_k$
% %             \State Augment perception $\Tilde{\mathcal{O}}_i(x_i,\Tilde{S}_i)$
% %             \EndFor
% %         \EndFor
% %     % \EndFor
% % \end{algorithmic}
% % \label{alg:AugPerception}
% % \end{algorithm}


% % \subsection{Scan Match}
% % We assume that the NDT method subdivides the surrounding space uniformly into cells small enough so that each cell will contain at most one point of the observation. In this case, if a cell contains the point $q^{\prime},$ then the corresponding normal distribution will have mean $q = q^{\prime}.$ Thus, the scan match of the same observation $\mathcal{O}(\mathbf{x}_1, S_1)$ is $n_s,$ which means $r = 0$ and $\mathcal{L}_s(r) = n_s$.



\subsection{Impact of Attacks}
\label{subsec:impact-of-attacks}
We now describe how each of the attacks defined in Section~\ref{subsec:threat-model} affects the obstacle detection algorithm of Section~\ref{subsec:occupied-area-identification}. These attack impacts will motivate the development of our FDII algorithm. In what follows, we let A denote the index of the attacked vehicle.

% Since different attacks have different abilities and purposes, the impacts of the attacks on the observations and occupied areas are also different. %We conclude the impacts in the following table for later analysis. 
% \begin{table}[]
%     \centering
%     \begin{tabular}{ |c|c|c|c|c|c|c| } 
%      \hline
%      Attack & $\mathcal{O}(x_A, S_A)$ & $\mathcal{O}^b_k(x_A, S_A)$ & $\mathcal{U}_A$ & $\mathcal{O}(x_A, S_B)$ & $\mathcal{O}^b_k(x_A, S_B)$ & $\mathcal{U}_B$\\ 
%      \hline
%      a & move & up & up & - & - & -  \\ 
%      b1 & move & move & up & - & - & - \\ 
%      b2 & move & move & up & - & - & - \\
%      b3 & move & move & up & - & - & - \\
%      c & unch & unch & unch & unch & unch & unch \\
%      \hline
%     \end{tabular}
%     \caption{Impacts of Attacks on Observations and Occupied Areas}
%     \label{tab:impacts-of-attacks}
% \end{table}

% For \textcolor{blue}{Attack NEO}, the points of observation $\mathcal{O}(x_A, S_A)$ of the compromised LiDAR are changed, which introduces $\mathcal{O}^b_k(x_A, S_A)$ and corresponding $\mathcal{U}_A$. For \textcolor{blue}{Attack PRA}1, b2, and b3, the $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}^b_k(x_A, S_A)$ corresponding to the original obstacle are changed to fail the LiDAR detection algorithm. In order to achieve that, $\mathcal{U}_A$ has to be enlarged to fully cover the original obstacle. For \textcolor{blue}{Attack AO}, $\mathcal{O}(x, S)$, $\mathcal{O}^b_k(x, S)$, and $\mathcal{U}$ are unchanged for all compromised LiDAR sensors.

\underline{\textit{For Attack NEO}}, the artificial points $e^{\prime}$ introduce a fake obstacle with points $\mathcal{O}^b_k(x_A, S_A)$. Since there is only one victim, we have $\mathcal{O}^b_k(x_A, S_A) \nsubseteq \mathcal{U}_B$. Since there is no true obstacle, we have $\mathcal{U}_B = \emptyset$.

\underline{\textit{For Attack PRA1}}, the artificial points $e^{\prime}$ introduce fake $\mathcal{O}^b_k(x_A, S_A)$. There is a true obstacle, so $\mathcal{U}_B \neq \emptyset.$ In this case, since Agent B could observe the full space of $\mathcal{O}^b_k(x_A, S_A)$, we have $\mathcal{O}^b_k(x_A, S_A) \nsubseteq \mathcal{U}_B$ and $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B = \emptyset.$ 

\underline{\textit{For Attack PRA2}}, there are also fake $\mathcal{O}^b_k(x_A, S_A)$ and non-empty $\mathcal{U}_B$. However, $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \nsubseteq \mathcal{U}_B$ and $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B \neq \emptyset$ in this case because Agent B could only observe the partial space of $\mathcal{O}^b_k(x_A, S_A)$. 

\underline{\textit{For Attack PRA3}}, the fake $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ is fully covered by non-empty $\mathcal{U}_B$ because Agent B could not observe the space of $\mathcal{O}^b_k(x_A, S_A)$, which means $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \subseteq \mathcal{U}_B$. 

\underline{\textit{For Attack AO and the true obstacle}}, there is non-empty $\mathcal{O}^b_k(x_A, S_A)$ and non-empty $\mathcal{U}_B$ corresponding to the adversarial object and the true obstacle, respectively. According to Lemma~\ref{lemma:occupied-area-covers-obstacle-projection}, we have $\mathcal{P}(P^{ob}) \subseteq \mathcal{U}_B.$ Since $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \subseteq \mathcal{P}(P^{ob})$, we have $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \subseteq \mathcal{U}_B$.
 
% b2, and b3, the $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}^b_k(x_A, S_A)$ corresponding to the original obstacle are changed to fail the LiDAR detection algorithm. In order to achieve that, $\mathcal{U}_A$ has to be enlarged to fully cover the original obstacle. For \textcolor{blue}{Attack AO}, $\mathcal{O}(x, S)$, $\mathcal{O}^b_k(x, S)$, and $\mathcal{U}$ are unchanged for all compromised LiDAR sensors. 

% \begin{table}[]
%     \centering
%     \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%      \hline
%      Attack & $\mathcal{P}(\mathcal{O}(x_A, S_A))$ & $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ & $\mathcal{U}_A$ & $\Tilde{\mathcal{O}}_1$ & $\Tilde{\mathcal{O}}_2$ & $\Tilde{\mathcal{O}}_3$ & $\Tilde{\mathcal{O}}_4$\\ 
%      \hline
%      a & move & up & up & unch & up & unch & up \\ 
%      b1 & move & move & up & down & up & down & up \\ 
%      b2 & move & move & up & down & change & down & up \\
%      b3 & move & move & up & down & down & down & up \\
%      c & unch & unch & unch & unch & unch & unch & unch \\
%      \hline
%     \end{tabular}
%     \caption{Decision Table}
%     \label{tab:my_label}
% \end{table}
 


\subsection{Fault Detection, Identification, and Isolation}
\label{sec:FDII}
The objective of the proposed fault detection, identification, and isolation (FDII) algorithm is to detect the mismatch between the augmented observations of different agents, identify the spoofed agent, isolate the corrupted parts of the raw data, and restore the true unsafe region. The proposed FDII algorithm is illustrated as Fig.~\ref{fig:FDII}.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figs/decision_tree.png}
    \caption{Decision tree of the FDII algorithm.}
    \label{fig:FDII}
\end{figure}

% \begin{table}[]
%     \centering
%     \begin{tabular}{ |c|c|c|c| } 
%      \hline
%      Type of Attack & detect i & $U_i$ Non-Empty & Scan Match \\ 
%      \hline
%      None True & T & T & T \\ 
%      None False & F & F & - \\ 
%      a & T & T & F \\ 
%      b1, b2 & F & T & F \\ 
%      b3, c & F & T & T \\
%      \hline
%     \end{tabular}
%     \caption{Decision Table}
%     \label{tab:my_label}
% \end{table}

The intuition is that if the LiDAR observation of Agent A is spoofed by the adversary, the artificial points $e^{\prime}$ will not match the data collected by another agent $B \neq A$, $B \in L$. $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B$ is equal to the set of points that are observed by Agent A and are in the space that can be observed by Agent B. We check whether $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B$ is empty as follow. We traverse the point $p \in \mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ to see whether $p$ satisfies $h_l(x) - \zeta_h \leq 0, \forall l \in \{1,\ldots,n^h_{Bk}\}.$ If not, we put $p$ into $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B$. We name this operation a scan match.
% We limit the scope of scan match of the observation to the set $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B$, which is equal to the set of points that are observed by Agent A and are in the space that can be observed by Agent B. 
% We also limit the scope of scan match of the observation to the horizontal axes of two augmented observations $\Tilde{\mathcal{O}}_a^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_b^{\mathcal{I}}$. 

% If it is a 2-D LiDAR, we use $\Tilde{\mathcal{O}}_i^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_j^{\mathcal{I}}$. If it is a 3-D LiDAR, we use the values of x and y coordinates of $\Tilde{\mathcal{O}}_i^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_j^{\mathcal{I}}$, which means the projection of the scan on the horizontal plane. 

% Since the proposed method is based on the extra LiDAR observation, We  assume that $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap (I_B \setminus \cup(\mathcal{U}_B \setminus \mathcal{P}(\mathcal{O}^b_k(x_A, S_B)))) \neq \emptyset,$ which means that Agent B can observe at least a part of the area of the obstacle which Agent A observes. 

% Since the proposed method is based on the extra LiDAR observation, we limit the range of fault detection as $\mathcal{I}_A \cap \mathcal{I}_B.$ We further assume that the 

% The following lemma guarantees the detection of the attack if the spoofer presents.

% The following lemma guarantees the detection of the mismatch between observations even if the spoofer presents.

\begin{lemma}
    \label{lemma:scan-match}
    % Suppose Agent A observes obstacle with observation $\mathcal{O}^b_k(x_A, S_A)$ and receives $\mathcal{U}_B$ from Agent B. 
    If $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B \neq \emptyset,$ then Agent A is being targeted by an attack of type NEO, PRA1, or PRA2. If $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B = \emptyset,$ then either Obstacle $k$ is a true obstacle, or Agent A is under Attack PRA3 or AO.
\end{lemma}

\begin{proof}
    We first consider $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B \neq \emptyset.$ We have $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B =\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B) \neq \emptyset$, which implies $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \neq (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B).$ Thus, we have $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \nsubseteq \mathcal{U}_B.$
    % \begin{align*}
    %     &\quad\quad\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B \\
    %     &=\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B) \neq \emptyset \\
    %     &\Rightarrow \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \neq (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B) \\
    %     &\Rightarrow \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \nsubseteq \mathcal{U}_B
    % \end{align*}
    According to Section.~\ref{subsec:impact-of-attacks}, if $\mathcal{U}_B = \emptyset$, Attack NEO occurs. If $\mathcal{U}_B \neq \emptyset$, Attack PRA1 or PRA2 occurs.

    We next consider $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B = \emptyset.$ We have $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B =\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B) = \emptyset,$ which means $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) = (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B).$ Thus, we have $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \subseteq \mathcal{U}_B.$
    % \begin{align*}
    %     &\quad\quad\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B \\
    %     &=\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B) = \emptyset \\
    %     &\Rightarrow \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) = (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B) \\
    %     &\Rightarrow \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \subseteq \mathcal{U}_B
    % \end{align*}
    According to Section~\ref{subsec:impact-of-attacks}, either there is a true obstacle or Attack PRA3 or Attack AO occurs.
\end{proof}

% \begin{lemma}
%     Suppose Agent A may be under attack and Agent B is safe. If \textcolor{blue}{Attack NEO}, b1, or b2 occurs, then $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B \neq \emptyset.$ If there is a true obstacle or \textcolor{blue}{Attack PRA}3 or \textcolor{blue}{Attack AO} occurs, then $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B = \emptyset.$
% \end{lemma}

% \begin{proof}
%     For \textcolor{blue}{Attack NEO}, $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) = \mathcal{P}(e^{\prime})$ and $\mathcal{U}_B = \emptyset.$ We have $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B = \mathcal{P}(e^{\prime}) \setminus \emptyset = \mathcal{P}(e^{\prime}).$

%     For \textcolor{blue}{Attack PRA}1, $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) = \mathcal{P}(e^{\prime})$ and $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B = \emptyset.$ We have $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B = \mathcal{P}(e^{\prime}) \setminus (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B) = \mathcal{P}(e^{\prime}) \setminus \emptyset = \mathcal{P}(e^{\prime}).$

%     For \textcolor{blue}{Attack PRA}2, $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) = \mathcal{P}(e^{\prime})$ and $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B \neq \emptyset.$ We have $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \setminus \mathcal{U}_B = \mathcal{P}(e^{\prime}) \setminus \mathcal{U}_B.$

%     For \textcolor{blue}{Attack PRA}3, 
% \end{proof}

% \begin{lemma}
% Suppose the object detection algorithms of Agent A outputs the bounding boxes $\mathcal{B}_A$ and the obstacle set $\mathcal{O}^b_k(x_A, S_A)$ inside $\mathcal{B}_A$. Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied areas $\mathcal{U}_A$ and $\mathcal{U}_B$ of Agent A and Agent B, respectively, and the obstacle set $\mathcal{O}^b_k(x_A, S_B)$ which has $\mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \subseteq \mathcal{U}_A$. If $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then either there exists a true obstacle in $\mathcal{B}_A$ or \textcolor{blue}{Attack PRA}3/c occurs. Otherwise, Agent A is under \textcolor{blue}{Attack NEO} or \textcolor{blue}{Attack PRA}1/b2. 
% \end{lemma}

% \begin{proof}
%     We first show that if neither there exists a true obstacle in $\mathcal{B}_A$ nor \textcolor{blue}{Attack PRA}3/c occurs, which means either \textcolor{blue}{Attack NEO} or \textcolor{blue}{Attack PRA}1/b2 occur, then $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \neq n_s$. We consider two cases, namely (i) there exists a falsified obstacle and (ii) there exists \textcolor{blue}{Attack PRA}1 or \textcolor{blue}{Attack PRA}2 which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$.

%     \textit{Case (i):} In this case, Agent A is under \textcolor{blue}{Attack NEO} and we have $\mathcal{U}_A \neq \emptyset$ and $\mathcal{U}_B = \emptyset.$ Since there is only one attack, Agent B is attack-free and $\mathcal{O}^b_k(x_A, S_B) = \emptyset.$ According to Eq.~\eqref{eq:augmented-perception-A} and~\eqref{eq:augmented-perception-B}, the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     =& \{\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))\cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B))\\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}\\
%     =&\{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}
% \end{align*}

%     Since $\Tilde{\mathcal{O}}(x_A, S_A) \neq \Tilde{\mathcal{O}}(x_A, S_B),$ the extra term $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ in $\Tilde{\mathcal{O}}(x_A, S_A)$ will introduce difference in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$

%     \textit{Case (ii):} In this case, $\mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \subseteq \mathcal{U}_A$. However, $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ is not a subset of $\mathcal{U}_B$, which means that there exist elements in $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ that is also elements in $\mathcal{I}_B \setminus \mathcal{U}_B$. The augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follows.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B))\\
%     &\cup (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B ) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
% \end{align*}

%     Since there exist elements in $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ that is not in $\mathcal{U}_B$, we have $(\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B) \subseteq \mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ and there are more points in $\Tilde{\mathcal{O}}(x_A, S_A)$ than in $\Tilde{\mathcal{O}}(x_A, S_B)$. This will introduce differences in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$

%     In both Case (i) and Case (ii), we have $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \neq n_s$, which proves that if neither there exists a true obstacle in $\mathcal{B}_A$ nor \textcolor{blue}{Attack PRA}3/c occurs, then $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \neq n_s$. Hence, the converse-negative proposition that 'if $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then either there exists a true obstacle in $\mathcal{B}_A$ or \textcolor{blue}{Attack PRA}3/c occurs' holds as well.

%     Next, we show that if neither Attack 1 nor \textcolor{blue}{Attack PRA}1/b2 occurs, which means that either there exists a true obstacle in $\mathcal{B}_A$ or \textcolor{blue}{Attack PRA}3/c occurs, then $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$. In both cases, according to Eq.~\eqref{eq:augmented-perception-A} and~\eqref{eq:augmented-perception-B}, the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
%     \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B))\\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
%     \end{align*}

%     Since $\Tilde{\mathcal{O}}(x_A, S_A) = \Tilde{\mathcal{O}}(x_A, S_B),$ we have $r = 0$ and $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, which proves that if neither Attack 1 nor \textcolor{blue}{Attack PRA}1/b2 occurs, then $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$. Hence, the converse-negative proposition that 'if $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \neq n_s$, then either Attack 1 or \textcolor{blue}{Attack PRA}1/b2 occurs' holds as well.
% \end{proof}

% \begin{lemma}
% Suppose the object detection algorithms of Agent A outputs the bounding boxes $\mathcal{B}_A$ and the obstacle set $\mathcal{O}^b_k(x_A, S_A)$ inside $\mathcal{B}_A$. Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied areas $\mathcal{U}_A$ and $\mathcal{U}_B$ of Agent A and Agent B, respectively, and the obstacle set $\mathcal{O}^b_k(x_A, S_B)$ which has $\mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \subseteq \mathcal{U}_A$. If $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then there exists a true obstacle in $\mathcal{B}_A$. Otherwise, Agent A is under \textcolor{blue}{Attack NEO}. 
% % Suppose the object detection algorithms of Agent A outputs the bounding boxes $\mathcal{B}_A$. Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied area $\mathcal{U}_A$ and $\mathcal{U}_B,$ the sets of projection of the points inside $\mathcal{B}_A$ on the horizontal plane $O_A,$ and the set of projection of $O_B$, If the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ match, then there exists a true obstacle
% % Suppose the object detection algorithms of Agent A and B output the bounding boxes $\mathcal{B}_A$ and $\mathcal{B}_B$ for the same obstacle, respectively. Given the sets of projection of the points inside $\mathcal{B}_A$ and $\mathcal{B}_B$ on the horizontal plane $O_A$ and $O_B$, the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, and the occupied area $\mathcal{U}_A$ and $\mathcal{U}_B.$ If the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ match, then there exists a true obstacle

% \end{lemma}

% \begin{proof}
% We consider two cases, namely (i) there exists a true obstacle in $\mathcal{B}_A$ and (ii) there exists a falsified obstacle.

% \textit{Case (i):} In this case, the spoofer does not present. We calculate the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate as follow.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B))\\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
% \end{align*}

% Since $\Tilde{\mathcal{O}}(x_A, S_A) = \Tilde{\mathcal{O}}(x_A, S_B),$ we have $r = 0$ and $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s.$

% \textit{Case (ii):} In this case, Agent A is under \textcolor{blue}{Attack NEO} and we have $\mathcal{U}_A \neq \emptyset$ and $\mathcal{U}_B = \emptyset.$ Since there is only one attack, Agent B is attack-free and $\mathcal{O}^b_k(x_A, S_B) = \emptyset.$ The augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     =& \{\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))\cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B))\\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}\\
%     =&\{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}
% \end{align*}

% Since $\Tilde{\mathcal{O}}(x_A, S_A) \neq \Tilde{\mathcal{O}}(x_A, S_B),$ the extra term $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ in $\Tilde{\mathcal{O}}(x_A, S_A)$ will introduce difference in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$

% % \textit{Case (i):} In this case, the spoofer does not present. We calculate the scan match $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B)$ as follow.
% % \begin{align*}
% %     &\quad\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) \\
% %     &= \{((\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}_\mathcal{B}(x_A, S_A)) \\
% %     &\quad\cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A))\}\\ 
% %     &\ominus ((Ground_B\cap U_A)\cup O_B\cup (e^{\prime}\cup Ground_A\cap U_B))
% % \end{align*}
% \end{proof}


% \begin{lemma}
% Suppose there exists the obstacle set $\mathcal{O}^b_k(x_A, S_A)$ with the occupied area $\mathcal{U}_A$, and the object detection algorithms of Agent A does not detect any obstacle with vertical projection in $\mathcal{U}_A$.
% Given the observations $\mathcal{O}(x_A, S_A)$ and $\mathcal{O}(x_A, S_B)$, the occupied areas $\mathcal{U}_A$ and $\mathcal{U}_B$ of Agent A and Agent B, respectively, and the obstacle set $\mathcal{O}^b_k(x_A, S_B)$ which has $\mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \subseteq \mathcal{U}_A$. If $\Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s$, then there exists \textcolor{blue}{Attack PRA}3 or \textcolor{blue}{Attack AO} which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$. Otherwise, there exists \textcolor{blue}{Attack PRA}1 or \textcolor{blue}{Attack PRA}2 which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$. 
% \end{lemma}

% \begin{proof}
% We consider two cases, namely (i) there exists \textcolor{blue}{Attack PRA}3 or \textcolor{blue}{Attack AO} which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$, and (ii) there exists \textcolor{blue}{Attack PRA}1 or \textcolor{blue}{Attack PRA}2 which leaves the trace in the observation $\mathcal{O}(x_A, S_A)$ with vertical projection in $\mathcal{U}_A$.

% \textit{Case (i):} In this case, $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \subseteq \mathcal{U}_B$ and $\mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \subseteq \mathcal{U}_A$. We calculate the augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate as follow.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B))\\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
% \end{align*}

% Since $\Tilde{\mathcal{O}}(x_A, S_A) = \Tilde{\mathcal{O}}(x_A, S_B),$ we have $r = 0$ and $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) = n_s.$

% \textit{Case (ii):} In this case, $\mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \subseteq \mathcal{U}_A$. However, $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ is not a subset of $\mathcal{U}_B$, which means that there exist elements in $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ that is also elements in $\mathcal{I}_B \setminus \mathcal{U}_B$. The augmented perceptions $\Tilde{\mathcal{O}}(x_A, S_A)$ and $\Tilde{\mathcal{O}}(x_A, S_B)$ for Agent A and B in Agent A's coordinate are as follow.
% \begin{align*}
%     \Tilde{\mathcal{O}}(x_A, S_A) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \\
%     &\cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B)) \cup (\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A)\}\\
%     \Tilde{\mathcal{O}}(x_A, S_B) =& \{(\mathcal{P}(\mathcal{O}(x_A, S_B)) \cap \mathcal{U}_A) \cup \mathcal{P}(\mathcal{O}^b_k(x_A, S_B))\\
%     &\cup (\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B ) \cup (\mathcal{P}(\mathcal{O}(x_A, S_A)) \cap \mathcal{U}_B)\}
% \end{align*}

% Since there exist elements in $\mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ that is not in $\mathcal{U}_B$, we have $(\mathcal{P}(\mathcal{O}^b_k(x_A, S_A)) \cap \mathcal{U}_B) \subseteq \mathcal{P}(\mathcal{O}^b_k(x_A, S_A))$ and there are more points in $\Tilde{\mathcal{O}}(x_A, S_A)$ than in $\Tilde{\mathcal{O}}(x_A, S_B)$. This will introduce difference in the scan match. Thus, we will have $\mathcal{L}_s(r) = \Tilde{\mathcal{O}}(x_A, S_A) \ominus \Tilde{\mathcal{O}}(x_A, S_B) < n_s.$
% \end{proof}

We design the decision tree as shown in Fig.~\ref{fig:FDII} to detect each attack. At each time, Agent A collects the current scans of nearby agents $S_j, \forall j \in L, j \neq A$. The corresponding observations $\mathcal{O}(x_A, S_j),$ the observations of obstacles $\mathcal{O}^b_k(x_A, S_j),$ and the occupied areas $\mathcal{U}_j$ are calculated by Agent A. For each bounding box provided by the object detection algorithm, Agent A does a scan match based on the result of Lemma~\ref{lemma:scan-match}. The points in the bounding box belong to either the non-existing obstacle from Attack NEO or the true obstacle. After detecting and identifying the attack or authenticating that it is the true obstacle, Agent A removes the points from the observation and discards the corresponding occupied area, then solves the next bounding box. After traversing all bounding boxes, Agent A checks whether there is still observation of the obstacle. If not, there is no more attack or obstacle. If there is the observation of the obstacle, there is an attack and a scan match will be done to decide the classification of the attack.

% We consider three LiDAR attacks presented in Sec.~\ref{subsec:threat-model} as shown in Fig.~\ref{fig:three-LiDAR-attacks}. Without loss of generality, we show the idea by using two agents.

% The following lemma shows that the unsafe region can be achieved even if the three LiDAR attacks occur.

% \begin{lemma}
%     decision tree
% \end{lemma}

% Based on the results of Lemma ..., we propose the function ... in Algorithm~... to generate unsafe regions that can be used to provide feasible control inputs to guarantee safety requirements.

% The rules to update unsafe regions based on multi-agent observations.
% \begin{enumerate}
%     \item If an occupied area is only observed by one agent, then it covers a falsified non-existing obstacle resulted from a relay attack.

%     \item If an occupied area 
% \end{enumerate}

% Only consider the intersection of occupied area when doing mismatch detection.
% \begin{enumerate}
%     \item For attack a and b1 (non-existing obstacle), the intersection is empty.

%     \item For \textcolor{blue}{Attack PRA}2 (Agent j could partically observe the area covered by Agent i's occupied area), we could narrow the range of the intersection based on the observation of Agent j.

%     \item For \textcolor{blue}{Attack PRA}3 and c (Agent j cannot observe the area covered by Agent i's occupied area), we append the intersection into the updated unsafe region.
% \end{enumerate}

% Challenges:
% \begin{enumerate}
%     \item How to identify the occupied area?

%     Divide the overlapping area of the observations $\Tilde{\mathcal{O}}_i(O_c,S_i)$ and $\Tilde{\mathcal{O}}_j(O_c,S_j)$ uniformly into small cells with constant size. If there is no point $p_i$ inside the cell, we consider the empty cell as a part of an occupied area of Agent $i$. The nearby empty cells combine together as an occupied area. The adjacent nonempty cells are considered as the boundary of the occupied area.

%     \item How to do augmented perception?

%     Do not need augmented perception in this case.

%     \item How to do mismatch detection?

%     Do not need to do mismatch detection in this case. 
% \end{enumerate}

% In Fig.~\ref{fig:RelayExp}, the spoofer falsifies a non-existing obstacle in the raw data of the attacked Agent $i$ by firing laser beams to the receiver of the LiDAR. The augment perception $\Tilde{\mathcal{O}}_i(O_c,\Tilde{S}_i)$ of Agent $i$ is obtained by combining points $\Tilde{p}_k$ in the overlapping area of the falsified occupied area $\mathcal{U}_i$ and the scan covered area $\mathcal{I}_j$. This overlapping area is guaranteed to exist and be the same as $\mathcal{U}_i$ by Eq.~\eqref{eq:jointpercept}. The augment perception $\Tilde{\mathcal{O}}_j(O_c,\Tilde{S}_j)$ of Agent $j$ is identical with the observation $\Tilde{\mathcal{O}}_j(O_c,S_j)$ because there is no occupied area in the raw data. Thus, there is mismatch of the observation in the overlapping area $\mathcal{I}_i\cap \mathcal{I}_j$ of two augmented observation $\Tilde{\mathcal{O}}_i^{\mathcal{I}}$ and $\Tilde{\mathcal{O}}_j^{\mathcal{I}}$.

% In Fig.~\ref{fig:PRAExp}, the spoofer implements PRA by creating a falsified obstacle between Agent $i$ and the true obstacle. Since the position of the falsified obstacle and the position of the true obstacle are different, there exists occupied area that can only be detected by one of the agent, which means $\mathcal{U}_i \neq \mathcal{U}_j$. According to Eq.~\eqref{eq:jointpercept}, $\mathcal{U}_i \subseteq \mathcal{I}_j$ and $\mathcal{U}_j \subseteq \mathcal{I}_i.$ Thus, $(\mathcal{I}_j \cap \mathcal{U}_i) = \mathcal{U}_i \neq \mathcal{U}_j = (\mathcal{I}_i \cap \mathcal{U}_j)$.

% In Fig.~\ref{fig:AdvObjExp}, 

% We compute relative pose by performing scan match $\Tilde{\mathcal{O}}_i^{\mathcal{I}} \ominus \Tilde{\mathcal{O}}_j^{\mathcal{I}}$. 

% \begin{proposition}
%     (Working on *proposition)
% \end{proposition}
% If the relative pose exceed a threshold derived by (*proposition), it means one of the scans is spoofed. We next identify the area affected spoofed data by solving the following optimization problem  
% \begin{equation}
%     \label{eq:FIdent}
%     \min_c (\Tilde{\mathcal{O}}_i^{\mathcal{I}} \backslash c)\ominus (\Tilde{\mathcal{O}}_j^{\mathcal{I}} \backslash c)
% \end{equation}
% With the mismatched area spotted, we then formulate decision tree to identify the attack type and spoofed agent. 

% (working on) train of thought: We summarize the symptom of different attack type and formulate the Decision tree 



% We finally proposed Alg. \ref{alg:FDII} to summarize the workflow. 
% % \begin{algorithm}[!htbp]
% % \caption{LiDAR Fault Detection, Identification and Isolation}
% % \begin{algorithmic}[1]
% %     \State \textbf{Input:} A set of augmented LiDAR Observation $\boldsymbol{\Tilde{\mathcal{O}}}:=\{\Tilde{\mathcal{O}},\forall i\in L\}$
% %     \State \textbf{Output:} 
% %     \For{$i,j\in L$}
% %         \State Compute $r \gets \Tilde{\mathcal{O}}_i^{\mathcal{I}} \ominus \Tilde{\mathcal{O}}_j^{\mathcal{I}}$
% %         \If{$r>\theta$}
% %             \State Solve \eqref{eq:FIdent}
% %             \State (Working on)
% %         \EndIf
% %     \EndFor
% % \end{algorithmic}
% % \label{alg:FDII}
% % \end{algorithm}

After detecting the scan mismatch and identifying the spoofed agent, the proposed FDII algorithm isolates the corrupted parts of the raw data and updates the unsafe region by extracting the intersection of the unions of the occupied areas of the agents indexed in $L.$ 

We calculate the intersection $\bigcap_j (\cup_k \mathcal{U}_{jk})$ of Agent $j$ as follows, where $j \in L$ is the index of the neighboring agents, $k \in \{1,\ldots,n^j_o\}$ is the index of the occupied areas of Agent $j,$ and $n^j_o$ is the number of the occupied areas of Agent $j.$ For a certain Agent $j \in L$, each $\mathcal{U}_{jk}, k \in \{1,\ldots,n^j_o\}$ corresponds to either a true obstacle or a non-existing obstacle resulting from Attack NEO. Each obstacle (including the true obstacles and the non-existing obstacles) is indexed as the set of points $P^{ob}_k, k \in \{1,\ldots,n^j_o\}.$ %We further denote the true obstacles and the non-existing obstacles as 
Suppose $L = \{A, B\}$ and $n^A_o = n^B_o = 2.$ Agent A calculates $\mathcal{U}_{A1}$, $\mathcal{U}_{A2}$, $\mathcal{U}_{B1}$, and $\mathcal{U}_{B2}$ based on $\mathcal{O}^b_k(x_A, S_A)$ and $\mathcal{O}^b_k(x_A, S_B)$. Boundaries $h^{A1}_l(x),$ $h^{A2}_l(x),$ $h^{B1}_l(x),$ and $h^{B2}_l(x)$ of $\mathcal{U}_{A1}$, $\mathcal{U}_{A2}$, $\mathcal{U}_{B1}$, and $\mathcal{U}_{B2}$ are computed. We traverse the scan points in $\mathcal{U}_{A1}$ and $\mathcal{U}_{A2}$ and check whether they satisfy either $h^{A1}_l(x)$ or $h^{A2}_l(x).$ If yes, we put the points in the union $\cup_k \mathcal{U}_{Ak}.$ $\cup_k \mathcal{U}_{Bk}$ can be calculated in a similar way. New boundaries $h^{A1}_{l^\prime}(x)$ and $h^{B1}_{l^\prime}(x)$ for the unions $\cup_k \mathcal{U}_{Ak}$ and $\cup_k \mathcal{U}_{Bk}$ are calculated. When calculating the intersection $\bigcap_j (\cup_k \mathcal{U}_{jk})$, we check whether the point in $\cup_k \mathcal{U}_{Ak}$ and $\cup_k \mathcal{U}_{Bk}$ satisfies both $h^{A1}_{l^\prime}(x)$ and $h^{B1}_{l^\prime}(x)$. If yes, we put it in the intersection $\bigcap_j (\cup_k \mathcal{U}_{jk})$. 

% Agent A calculates $\mathcal{U}_{A1}$, $\mathcal{U}_{A2}$, $\mathcal{U}_{B1}$, and $\mathcal{U}_{B2}$ based on $\mathcal{O}^b_k(x_A, S_A)$ and $\mathcal{O}^b_k(x_A, S_B)$. $\mathcal{U}_{A1}$, $\mathcal{U}_{A2}$, $\mathcal{U}_{B1}$, and $\mathcal{U}_{B2}$ are convex hulls composed of multiple half-planes. The half-planes are expressed as linear constraints. We traverse the points in $\mathcal{U}_{A1}$ and $\mathcal{U}_{A2}$ and check whether they satisfy either the set of constraints corresponding to $\mathcal{U}_{A1}$ or $\mathcal{U}_{A2}$. If the point satisfies either set of the constraints, we put it in the union $\cup_k \mathcal{U}_{Ak}.$ $\cup_k \mathcal{U}_{Bk}$ can be calculated in a similar way. When calculating the intersection $\bigcap_j (\cup_k \mathcal{U}_{jk})$, we check whether the point in $\cup_k \mathcal{U}_{Ak}$ and $\cup_k \mathcal{U}_{Bk}$ satisfies all constraints corresponding to $\cup_k \mathcal{U}_{Ak}$ and $\cup_k \mathcal{U}_{Bk}$. If yes, we put it in the intersection $\bigcap_j (\cup_k \mathcal{U}_{jk})$.

%Suppose there are $n_b$ obstacles in the area of $\cap_j \mathcal{I}_j, \forall j \in L.$ Each obstacle is indexed as the set of points $P^{ob}_l, \forall l \in \{1,\ldots,n_b\}.$ 
% Since there is only one relay adversary targeting on one victim agent, without loss of generality, we denote the victim agent as Agent 1 and the occupied area corresponding to the non-existing obstacle as $\mathcal{U}_{11}$ if \textcolor{blue}{Attack NEO} occurs.
% Since there is only one relay adversary targeting on one victim agent, without loss of generality, we denote the non-existing obstacle as $P^{ob}_{1}$ if \textcolor{blue}{Attack NEO} occurs.
The following theorem shows that the updated unsafe region $\bigcap_j (\cup_k \mathcal{U}_{jk})$ contains $\mathcal{P}(P^{ob}_k), \forall k \in \{1,\ldots,n^j_o\}, j \in L$. 
\begin{theorem}
If the occupied areas $\mathcal{U}_{jk}$ of Agent $j$, $\forall j \in L, k \in \{1,\ldots,n^j_o\}$ in the area of $\cap_j \mathcal{I}_j$ are given, then $\mathcal{P}(P^{ob}_k) \subseteq \bigcap_j (\cup_k \mathcal{U}_{jk}).$ %If \textcolor{blue}{Attack NEO} occurs, then the existence of $P^{ob}_{1}$ will not enlarge $\bigcap_j (\cup_k \mathcal{U}_{jk}).$
\end{theorem}

\begin{proof}
    For each obstacle $P^{ob}_k, \forall k \in \{1,\ldots,n^j_o\}$, we consider two cases, namely (i) there is another obstacle $P^{ob}_{k^\prime}$ between obstacle $P^{ob}_k$ and Agent $j, \forall j \in L$, and $P^{ob}_{k^\prime}$ partially or fully blocks $P^{ob}_k$ from Agent $j,$ and (ii) There is no $P^{ob}_{k^\prime}$ that blocks $P^{ob}_k$ from Agent $j.$

    \underline{\textit{Case (i)}}: In this case, there exists $k^{\prime} \in \{1,\ldots,n^j_o\}$ such that $\mathcal{P}(P^{ob}_k) \cap \mathcal{U}_{jk^{\prime}} \neq \emptyset.$ We divide $P^{ob}_k$ into two parts: $\mathcal{P}(P^{ob}_k) \cap \mathcal{U}_{jk^{\prime}}$ and $\mathcal{P}(P^{ob}_k) \setminus \mathcal{U}_{jk^{\prime}}.$ For $\mathcal{P}(P^{ob}_k) \cap \mathcal{U}_{jk^{\prime}}$, since $(\mathcal{P}(P^{ob}_k) \cap \mathcal{U}_{jk^{\prime}}) \subseteq \mathcal{U}_{jk^{\prime}} \subseteq \cup_k \mathcal{U}_{jk}, \forall j \in L$, we have $(\mathcal{P}(P^{ob}_k) \cap \mathcal{U}_{jk^{\prime}}) \subseteq \bigcap_j (\cup_k \mathcal{U}_{jk}).$ For $\mathcal{P}(P^{ob}_k) \setminus \mathcal{U}_{jk^{\prime}},$ according to Lemma~\ref{lemma:occupied-area-covers-obstacle-projection}, we have $(\mathcal{P}(P^{ob}_k) \setminus \mathcal{U}_{jk^{\prime}}) \subseteq \mathcal{U}_{jk} \subseteq \cup_k \mathcal{U}_{jk}, \forall j \in L$. Thus, we have $(\mathcal{P}(P^{ob}_k) \setminus \mathcal{U}_{jk^{\prime}}) \subseteq \bigcap_j (\cup_k \mathcal{U}_{jk}).$

    \underline{\textit{Case (ii)}}: In this case, $\mathcal{P}(P^{ob}_k) \cap \mathcal{U}_{jk^{\prime}} = \emptyset, \forall k^{\prime} \in \{1,\ldots,n^j_o\}.$ According to Lemma~\ref{lemma:occupied-area-covers-obstacle-projection}, we have $\mathcal{P}(P^{ob}_k) \subseteq \mathcal{U}_{jk} \subseteq \cup_k \mathcal{U}_{jk}, \forall j \in L$. Thus, we have $\mathcal{P}(P^{ob}_k \subseteq \bigcap_j (\cup_k \mathcal{U}_{jk}).$
    
    % According to Lemma~\ref{lemma:occupied-area-covers-obstacle-projection}, for each obstacle $\mathcal{P}(P^{ob}_k)$, $\mathcal{P}(P^{ob}_k) \subseteq \mathcal{U}_{jk}, \forall j \in L, k \in \{1,\ldots,n^j_o\}.$ This implies that $\mathcal{P}(P^{ob}_k) \subseteq \cup_k \mathcal{U}_{jk}, \forall j \in L.$ Since this holds $\forall j \in L,$ we have $\mathcal{P}(P^{ob}_k) \subseteq \bigcap_j (\cup_k \mathcal{U}_{jk}).$

    % If \textcolor{blue}{Attack NEO} occurs with non-existing obstacle $P^{ob}_{1}$, and the victim agent is Agent $A,$ then only $\mathcal{U}_{A1} \neq \emptyset.$ Thus, only $\cup_k \mathcal{U}_{Ak}$ is enlarged by the adversary. If $\mathcal{U}_{A1} \subseteq \bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L, j \neq A,$ then no other agent can provide redundant observation in the area $\mathcal{U}_{A1},$ and we cannot decrease or delete $\mathcal{U}_{A1}.$ Since $\mathcal{U}_{A1}$ has already been contained in $\bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L, j \neq A,$ $P^{ob}_{1}$ does not enlarge $\bigcap_j (\cup_k \mathcal{U}_{jk}).$ If $\mathcal{U}_{A1} \nsubseteq \bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L, j \neq A,$ then $\mathcal{U}_{A1} \setminus \bigcap_j (\cup_k \mathcal{U}_{jk}) \neq \emptyset, \forall j \in L, j \neq A,$ and the area $\mathcal{U}_{A1} \setminus \bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L, j \neq A$ will not be included in $\bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L,$ thus does not enlarge $\bigcap_j (\cup_k \mathcal{U}_{jk}).$
\end{proof}
% Since there is only one relay adversary targeting on one victim agent, without loss of generality, we denote the non-existing obstacle as $P^{ob}_{1}$ if \textcolor{blue}{Attack NEO} occurs.
% The following theorem shows that the updated unsafe region $\bigcap_j (\cup_k \mathcal{U}_{jk})$ contains the true unsafe region in $\mathcal{P}(P^{ob}_k), \forall k \in \{1,\ldots,n^j_o\}, j \in L$. 
% \begin{theorem}
% If the occupied areas $\mathcal{U}_{jk}$ of Agent $j$, $\forall j \in L, k \in \{1,\ldots,n^j_o\}$ in the area of $\cap_j \mathcal{I}_j$ are given, then $\mathcal{P}(P^{ob}_k) \subseteq \bigcap_j (\cup_k \mathcal{U}_{jk}).$ If \textcolor{blue}{Attack NEO} occurs, then the existence of $P^{ob}_{1}$ will not enlarge $\bigcap_j (\cup_k \mathcal{U}_{jk}).$
% \end{theorem}

% \begin{proof}
%     According to Lemma~\ref{lemma:occupied-area-covers-obstacle-projection}, for each obstacle $\mathcal{P}(P^{ob}_k)$ (including the true obstacles and the non-existing obstacles), $\mathcal{P}(P^{ob}_k) \subseteq \mathcal{U}_{jk}, \forall j \in L, k \in \{1,\ldots,n^j_o\}.$ This implies that $\mathcal{P}(P^{ob}_k) \subseteq \cup_k \mathcal{U}_{jk}, \forall j \in L.$ Since this holds $\forall j \in L,$ we have $\mathcal{P}(P^{ob}_k) \subseteq \bigcap_j (\cup_k \mathcal{U}_{jk}).$

%     If \textcolor{blue}{Attack NEO} occurs with non-existing obstacle $P^{ob}_{1}$, and the victim agent is Agent $A,$ then only $\mathcal{U}_{A1} \neq \emptyset.$ Thus, only $\cup_k \mathcal{U}_{Ak}$ is enlarged by the adversary. If $\mathcal{U}_{A1} \subseteq \bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L, j \neq A,$ then no other agent can provide redundant observation in the area $\mathcal{U}_{A1},$ and we cannot decrease or delete $\mathcal{U}_{A1}.$ Since $\mathcal{U}_{A1}$ has already been contained in $\bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L, j \neq A,$ $P^{ob}_{1}$ does not enlarge $\bigcap_j (\cup_k \mathcal{U}_{jk}).$ If $\mathcal{U}_{A1} \nsubseteq \bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L, j \neq A,$ then $\mathcal{U}_{A1} \setminus \bigcap_j (\cup_k \mathcal{U}_{jk}) \neq \emptyset, \forall j \in L, j \neq A,$ and the area $\mathcal{U}_{A1} \setminus \bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L, j \neq A$ will not be included in $\bigcap_j (\cup_k \mathcal{U}_{jk}), \forall j \in L,$ thus does not enlarge $\bigcap_j (\cup_k \mathcal{U}_{jk}).$
% \end{proof}

After calculating the updated unsafe region $\bigcap_j (\cup_k \mathcal{U}_{jk})$, we generate the convex hull for $\bigcap_j (\cup_k \mathcal{U}_{jk})$ and transfer the vertices of the convex hull to the safe controller. The safe controller restores the constraints $h^k_l(x), l = \{1,\ldots,n^h_k\}$ based on the vertices, where $h^k_l(x) > 0$ describes the corresponding half-plane and $n^h_k$ is the number of half-planes forming the convex hull $\mathcal{U}_{jk}$. We define $\Bar{h}_k(x) = \max_l -h^k_l(x)$.

% After calculating the updated unsafe region $\bigcap_j (\cup_k \mathcal{U}_{jk})$, we generate the convex hull for $\bigcap_j (\cup_k \mathcal{U}_{jk})$ and transfer the vertices of the convex hull to the safe controller. The safe controller restores the constraints $h_i(x), i = \{1,\ldots,n_h\}$ based on the vertices. 

% Theorem 2: prove that the intersection of the occupied areas contains the true unsafe region
% \begin{enumerate}
%     \item Input: the occupied area of Agent A $\mathcal{U}_A$ and Agent B $\mathcal{B}$

%     \item Output: the updated unsafe region (based on Lemma 1)
% \end{enumerate}

% \begin{lemma}
%     If the occupied areas $\mathcal{U}_A$ of Agent A and $\mathcal{U}_B$ of Agent B are given, then the updated unsafe region $\mathcal{U}_A \cap \mathcal{B}$ contains the true unsafe region $\mathcal{P}(P^{ob})$.
% \end{lemma}


% \subsection{Safety Region Estimation}
\subsection{Safe Control}
% \input{sections/control.tex}
\input{sections/control_v1.tex}
% We next design a safe control methodology to ensure safety of the controlled agent with desired probability. We formulate it as a control of a hybrid system. 

% In section \ref{sec:FDII}, we detect and estimate the obstacle to acquire unsafe region $h_1(x)$. Hence, we have the safe set as $\mathcal{C}_1:=\{x\mid h_1(x)\geq0\}$. 

==> sections/control.tex <==
% We next design a safe control methodology to ensure safety of the controlled agent with desired probability. We formulate it as a control of a hybrid system. 

% In section \ref{sec:FDII}, we detect and estimate the obstacle to acquire unsafe region $h_1(x)$. Hence, we have the safe set as $\mathcal{C}_1:=\{x\mid h_1(x)\geq0\}$. 

\textbf{Controller Formulation}
% controller candidates:
% AQR

% MPC
% pro:
%     can impose constraints on system state and control input
%     work for nonlinear system (may need linearization)
%     reoptimize the control input at every time step (we need to reoptimize the strategy every time we update the unsafe region)
%     can modify control input if state deviates or dynamics changes
% con:
%     optimize online

% Need gain-scheduled MPC for time-varying number of constraints

Model Predictive Control with Discrete-Time Control Barrier Function~\cite{zeng2021safety}

Reason to use MPC:
\begin{enumerate}
    \item nonlinear system dynamics (affine)

    \item constraints are changing over time (updated unsafe region from FDII) 
\end{enumerate}

\begin{align}
    \label{eq:objective-equation}
    \min_{u[t:t+T-1]} \ & (x[t+T]-x_r)^TF(x[t+T]-x_r) \\
    &+ \sum_{k=t}^{t+T-1} (x[k]-x_r)^TQ(x[k]-x_r) + u[k]^TRu[k] \nonumber\\
    \text{s.t.} \ & h_i(x[k+1])-h_i(x[k]) \geq -\gamma h_i(x[k]), \nonumber\\
    \label{eq:DT-CBF}
    & k = t,\cdots,t+T-1, \ i = 1,\cdots,n_h \\
    \label{eq:system-dynamics-equation}
    & x[k+1] = f(x[k]) + g(x[k]) u[k], k = t,\cdots,t+T-1 \\
    \label{eq:admissible-equations}
    & x[k] \in X, u[k] \in U, k = t,\cdots,t+T-1 
\end{align}
where $T$ is the prediction horizon, Eq.~\eqref{eq:objective-equation} means that we would like the vehicle to converge to the mid line of the lane ($x_r$) with less control effect, Eq.~\eqref{eq:DT-CBF} is the collection of the DT-CBFs corresponding to the unsafe regions provided by FDII, $n_h$ is the number of DT-CBF, Eq.~\eqref{eq:system-dynamics-equation} is the system dynamics, and Eq.~\eqref{eq:admissible-equations} are the admissible sets of system state $x$ and control input $u$. 

\begin{enumerate}
    \item Once FDII sends updated unsafe region, Eq.~\eqref{eq:DT-CBF}\eqref{eq:admissible-equations} will be updated accordingly.

    \item The optimization could be solved by using IPOPT solver. (https://coin-or.github.io/Ipopt/)
    
    \item \textbf{Design admissible sets $X$ and $U$}

        Objective: make sure that the vehicle always has enough braking distance.

        Idea: $u$ satisfies a function of the distance between the vehicle and the obstacle.

        Proof: safety and feasibility. 

        If $u \in U,$ there exists a feasible solution of $u$ that make the system state stays in the safe region.

        Challenge: may need to use a specific vehicle model instead of the general affine model. Otherwise, it is hard to design the admissible sets.

    \item \textbf{Proof of the safety between two time steps?}

        \cite{zeng2021safety} did not investigate this property.

        Shall we prove it or assume that the sample time is small enough?
\end{enumerate}

\newpage
\subsubsection{Ackermann steering model}
\begin{equation*}
    \begin{bmatrix} 
    \Dot{\phi}\\
    \Dot{x}\\
    \Dot{y}\\
    \Dot{\psi}\\
    \end{bmatrix}
    = \begin{bmatrix}
    (\tan \psi)/l & 0 \\
    \cos{\phi} & 0 \\
    \sin{\phi} & 0 \\
    0 & 1 \\
    \end{bmatrix} \begin{bmatrix}
        \nu\\
        \omega
    \end{bmatrix}
\end{equation*}
where $\phi$ is the heading angle between the orientation and the x-axis, $(x, y)$ is the position of the point between the rear wheels, $\psi$ is the steering angle of the imaginary steering wheel, $\nu$ is the forward velocity, and $\omega$ is the rate of turning the imaginary steering wheel.

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.5]{figs/Ackermann.png}
    \caption{Ackermann kinematic model}
    \label{fig:Ackermann}
\end{figure}

\subsubsection{diff-drive robot model}
\begin{equation*}
    \begin{bmatrix} 
    \Dot{\phi}\\
    \Dot{x}\\
    \Dot{y}\\
    \Dot{\theta}_L\\
    \Dot{\theta}_R\\
    \end{bmatrix}
    = \begin{bmatrix}
    -r/2d & r/2d \\
    \frac{r}{2}\cos{\phi} & \frac{r}{2}\cos{\phi} \\
    \frac{r}{2}\sin{\phi} & \frac{r}{2}\sin{\phi} \\
    1 & 0 \\
    0 & 1 \\
    \end{bmatrix} \begin{bmatrix}
        u_L\\
        u_R
    \end{bmatrix}
\end{equation*}
where $\phi$ is the heading angle between the orientation and the x-axis, $(x, y)$ is the position of the point between the independent wheels, $\theta$ is the rolling angle, and $u$ is the wheel velocity.

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.5]{figs/diff-drive-robot.png}
    \caption{Diff-drive robot model}
    \label{fig:diff-drive-robot}
\end{figure}


\subsubsection{Bicycle kinematic model}
\begin{equation*}
    \begin{bmatrix} 
    \Dot{\phi}\\
    \Dot{x}\\
    \Dot{y}\\
    \end{bmatrix}
    = \begin{bmatrix}
    0 & 1 \\
    \cos{\phi} & 0 \\
    \sin{\phi} & 0 \\
    \end{bmatrix} \begin{bmatrix}
        \nu\\
        \hat{\omega}
    \end{bmatrix}
\end{equation*}
where $\phi$ is the heading angle between the orientation and the x-axis, $(x, y)$ is the position of the point between the rear wheels, $\nu$ is the forward velocity, and $\hat{\omega}$ is the rate of heading angle.

Simplification of Ackermann steering model. Use the steering angle $\psi$ rather than the rate of the steering angle as input. Use $\hat{\omega} = \frac{v}{l}(\tan \psi)$ rather than $\psi$ as input. Based on the assumption that the rate of the steering angle is large enough so that the steering angle $\psi$ can be reached almost instantaneously. 

Discrete bicycle kinematic model is used in~\cite{yin2020nonlinear}.


\subsubsection{Dubin's car model}
\begin{equation*}
    \begin{bmatrix} 
    \Dot{\theta}\\
    \Dot{x}\\
    \Dot{y}\\
    \end{bmatrix}
    = \begin{bmatrix}
    \omega = \frac{v}{r_{turn}} \\
    \cos{\theta} \\
    \sin{\theta} \\
    \end{bmatrix} 
\end{equation*}
where $(x, y)$ is the position, $\theta$ is the orientation, $v$ is the velocity, $\omega$ is the angular velocity, and $r_{turn}$ is the radius of the curve.


\subsubsection{Design admissible set}

Intuition:

braking distance: $d = \frac{v^2}{2\mu g}$

Choose the minimum distance between the imaginary front wheel and the obstacle at the steering orientation as $d.$ We have the upper bound of velocity to avoid collision is $v = \sqrt{2\mu gd}$ 
